Learning Enriched Illuminants for Cross and Single Sensor Color Constancy

Color constancy aims to restore the constant colors of a scene under different illuminants. However, due to the existence of camera spectral sensitivity, the network trained on a certain sensor, cannot work well on others. Also, since the training datasets are collected in certain environments, the diversity of illuminants is limited for complex real world prediction. In this paper, we tackle these problems via two aspects. First, we propose cross-sensor self-supervised training to train the network. In detail, we consider both the general sRGB images and the white-balanced RAW images from current available datasets as the white-balanced agents. Then, we train the network by randomly sampling the artificial illuminants in a sensor-independent manner for scene relighting and supervision. Second, we analyze a previous cascaded framework and present a more compact and accurate model by sharing the backbone parameters with learning attention specifically. Experiments show that our cross-sensor model and single-sensor model outperform other state-of-the-art methods by a large margin on cross and single sensor evaluations, respectively, with only 16% parameters of the previous best model.

==> IEEEtran/subfiles/codeListingConfig.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%% CODE APPEARANCE CONFIG %%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%nicolas igor %%%%%%

%%%%%%%%%%%%%%%%% README %%%%%%%%%%%%%%%%%%%%
% This is a config file to set:
%   1. Style for listing package (could be use on any language)
%   2. Julia syntax highlighting definition
%   3. Command and environment to insert julia, python, and matlab code in your document easily.
%
%       a. new commands: \juliaFile, \pythonFile, and \matlabFile
%           All three are used like \juliaFile[folder_name]{file_name}
%           folder_name is optional, and do it with the slash, e.g. "myFolder/". When no folder is provided, it is assumed that the code is in the same directory as your document.
%           For file_name, do it without extension (it is assumed).
%       Example:
%           \juliaFile[codes/]{kMeans}
%           \juliaFile{randomForest}
%
%       b. new environments: if you want to write your code directly in your document. juliaText, pythonText, and matlabText are provided. Example:
%           \begin{juliaText}{Write your caption here.}
%           Write your code here
%           \end{juliaText}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



% Better font encoding, and customized fixed-width font
\usepackage[T1]{fontenc}
\usepackage{inconsolata}

% Colors Definition for Listing Highlighting 
\usepackage{color}
\definecolor{codeRed}{rgb}{0.5,0,0}
\definecolor{codeGreen}{rgb}{0,0.6,0}
\definecolor{codeBlue}{rgb}{0,0,0.5}
\definecolor{codeGray}{rgb}{0.5,0.5,0.5}
\definecolor{codeMauve}{rgb}{0.58,0,0.82}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%% LISTING FUN STARTS HERE!!! %%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{listings} % For displaying code

% General Appearance Settings in an Isolated Style
\lstdefinestyle{myStyle}{ %
  basicstyle=\small\ttfamily,      % the size of the fonts that are used for the code
  basewidth=0.5em,                 % sets size of reserved space on each column
  breakatwhitespace=true,          % sets if automatic breaks should only happen at whitespace
  breaklines=true,                 % sets automatic line breaking
  commentstyle=\color{codeGreen},  % comment style
  captionpos=b, 
  extendedchars=true,              % lets you use non-ASCII characters; for 8-bits encodings only, does not work with UTF-8
  frame=tb,	                       % adds a frame around the code
  keywordstyle=\color{codeBlue},       % keyword style
  numbers=left,                    % where to put the line-numbers; possible values are (none, left, right)
  numbersep=5pt,                   % how far the line-numbers are from the code
  numberstyle=\scriptsize\color{codeGray}, % the style that is used for the line-numbers
  rulecolor=\color{black},         % if not set, the frame-color may be changed on line-breaks within not-black text (e.g. comments (green here))
  showspaces=false,                % show spaces everywhere adding particular underscores; it overrides 'showstringspaces'
  showstringspaces=false,          % underline spaces within strings only
  showtabs=false,                  % show tabs within strings adding particular underscores
  stepnumber=1,                    % the step between two line-numbers. If it's 1, each line will be numbered
  numberfirstline=true, 
  numberblanklines=true,
  stringstyle=\color{codeMauve},     % string literal style
  tabsize=4,	                   % sets default tabsize to 4 spaces
}

% Definition of Julia Highlighting
\lstdefinelanguage{Julia}%
{ language = Matlab,% 
    keywordsprefix=\@,%
    morekeywords={
    exit,whos,edit,load,is,isa,isequal,typeof,tuple,ntuple,uid,hash,finalizer,convert,promote,
    subtype,typemin,typemax,realmin,realmax,sizeof,eps,promote_type,method_exists,applicable,
    invoke,dlopen,dlsym,system,error,throw,assert,new,Inf,Nan,pi,im,begin,while,for,in,return,
    break,continue,macro,quote,let,if,elseif,else,try,catch,end,bitstype,call,do,using,module,
    import,export,importall,baremodule,immutable,local,global,const,Bool,Int,Int8,Int16,Int32,
    Int64,Uint,Uint8,Uint16,Uint32,Uint64,Float32,Float64,Complex64,Complex128,Any,Nothing,nothing,
    function,type,typealias,abstract,case,false,otherwise,switch,true,include
  },%
  sensitive=true, %
  comment=[l]{\#}, % l is for line comment
  morecomment=[s]{\#=}{=\#}, % s is for start and end delimiter
  string=[b]" % defines that strings are enclosed in double quotes
}

% Command to include files of code easier, Julia
\newcommand{\juliaFile}[2][]{\lstinputlisting[caption=Script \emph{#2}., label=code:#2, style=myStyle, language=Julia]{#1#2.jl}}
% Command to include files of code easier, Python
\newcommand{\pythonFile}[2][]{\lstinputlisting[ label=code:#2, style=myStyle, language=Python]{#1#2.py}}
% Command to include files of code easier, Matlab
\newcommand{\matlabFile}[2][]{\lstinputlisting[caption=Script \emph{#2}., label=code:#2, style=myStyle, language=Matlab]{#1#2.m}}

% Environment to write by hand code easier, Julia
\lstnewenvironment{juliaText}[1]{\lstset{caption=#1, style=myStyle, language=Julia, firstnumber=1}}{}
% Environment to write by hand code easier, Python
\lstnewenvironment{pythonText}[1]{\lstset{caption=#1, style=myStyle, language=Python, firstnumber=1}}{}
% Environment to write by hand code easier, Matlab
\lstnewenvironment{matlabText}[1]{\lstset{caption=#1, style=myStyle, language=Matlab, firstnumber=1}}{}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%% LISTING FUN ENDED  %%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> IEEEtran/subfiles/conclusion.tex <==
\section{Conclusion}
In this paper, we propose a novel method to learn enriched illuminants for cross and single sensor CC. First, we present self-supervised cross-sensor training by unprocessing sRGB images to the RAW domain and correcting RAW images from multiple sensors. Second, we design a compact cascaded model by sharing the backbone in a cascaded network with a novel iteration-specific attention module learnt specifically. To further reduce the parameters, we design a lightweight head with two branches for both global and local feature learning. Without training on target-sensor data, the proposed model with our training method obtains state-of-the-art performance in the cross-sensor setting. Our model trained from scratch for single-sensor CC also shows superior performance on several popular benchmarks compared with other single-sensor CC methods. Furthermore, after fine-tuning our cross-sensor model on the target sensor, its performance improves further. 
%Besides current data augmentation methods, we also believe the synthesized samples can also benefits the training process, we will make it as the future work. 
%The proposed relighting method is pretty simple, and can be plugged into any other learning-based method with only several lines.

==> IEEEtran/subfiles/experiment.tex <==

\section{Experiments}
\label{sec:exp}
\begin{table*}[t]
    \small 
    \centering
    \caption{Comparison of angular errors with the state-of-the-art methods on the Gehler-Shi and NUS8 datasets. The \colorbox{lightgray!30}{shadowed} methods are for single-sensor evaluation while the others are for cross-sensor evaluation.}

    \begin{tabular}{l|c|ccccc|ccccc|c}
    \toprule
     \multirow{3}{*}{
     \diagbox{Method}{Angular Error}{Dataset}} & \multirow{3}{*}{Year} & \multicolumn{5}{c|}{Gehler-Shi} &\multicolumn{5}{c|}{NUS8} & \multirow{3}{*}{\#~Param.}\\
    \cline{3-12} 
    & &  Mean & Med. & Tri. & Best & Worst &  Mean & Med. & Tri. & Best & Worst \\
    & &   &  &  & 25\% & 25\% &   &  &  & 25\% & 25\%\\
    \hline
    Grey-World~\cite{gray-world} & 1980 & 6.36 & 6.28 & 6.28 & 2.33 & 10.58 & 4.59 & 3.46 & 3.81 & 1.16 & 9.85 & -\\
    White-Patch~\cite{white-patch} & 1986 & 7.55 & 5.68 & 6.35 & 1.45 & 16.12 & 9.91 & 7.44 & 8.78 & 1.44 & 21.27 & -\\
    SVR~\cite{SVR}& 2004 & 8.08 & 6.73 & 7.19 & 3.35 & 14.89 & - & - & - & - & - & - \\
    Shades-of-Gray~\cite{shades-of-gray}& 2004 & 4.93 & 4.01 & 4.23 & 1.14 & 10.20 & 3.40 & 2.57 & 2.73 & 0.77 & 7.41 & -\\
    1st-order Gray-Edge~\cite{gray-edge}& 2007 & 5.33 & 4.52 & 4.73 & 1.86 & 10.03 & 3.20 & 2.22 & 2.43 & 0.72 & 7.69 & -\\
    2nd-order Gray-Edge~\cite{gray-edge}& 2007 & 5.13 & 4.44 & 4.62 & 2.11 & 9.26 & 3.20 & 2.26 & 2.44 & 0.75 & 7.27 & - \\
    Bayesian~\cite{gehler2008bayesian} & 2008 & 4.82 & 3.46 & 3.88 & 1.26 & 10.49 & 3.67 & 2.73 & 2.91 & 0.82 & 8.21 & - \\
    Quasi-unsupervised~\cite{bianco2019quasi}& 2019 &  3.00 & 2.25 & - & - & - & 3.46 & 2.23 & - & - & - & 54.0M \\
    SIIE~\cite{siie} & 2019 & 2.77 &  1.93  & - & \textbf{0.55} & 6.53 & 2.05 & 1.50 & - & 0.52 & 4.48 & 1.8M \\
    Ours~(cross-sensor) &  2021 & \textbf{2.46} & \textbf{1.89} & \textbf{2.00} & 0.62 & \textbf{5.34} & \textbf{1.98} & \textbf{1.42} & \textbf{1.55} & \textbf{0.48} & \textbf{4.40} & 0.8M \\ \hline
    \rowcolor{lightgray!30} Corrected-Moment~\cite{Corrected-Moment}& 2013 & 2.86 & 2.04 & 2.22 & 0.70 & 6.34 & 2.95 & 2.05 & 2.16 & 0.59 & 6.89 & - \\
    \rowcolor{lightgray!30} Regression Tree~\cite{regression-tree}& 2015 & 2.42 & 1.65 & 1.75 & 0.38 & 5.87 & 2.36 & 1.59 & 1.74 & 0.49 & 5.54 & 31.5M \\
    \rowcolor{lightgray!30} CCC(dist+ext)~\cite{ccc}& 2015 & 1.95 & 1.22 & 1.38 & 0.35 & 4.76 & 2.38 & 1.48 & 1.69 & 0.45 & 5.85 & 0.7K \\
    \rowcolor{lightgray!30} DS-Net(HypNet+SeNet)~\cite{dsn} & 2016 & 1.90 & 1.12 & 1.33 & 0.31 & 4.84 & 2.24 & 1.46 & 1.68 & 0.48 & 6.08 & 5.3M \\
    \rowcolor{lightgray!30} FC4(SqueezeNet-FC4)~\cite{hu2017fc4} & 2017 & 1.65 & 1.18 & 1.27 & 0.38 & 3.78 & 2.23 & 1.57 & 1.72 & 0.47 & 5.15 & 1.7M \\
    \rowcolor{lightgray!30} FFCC(Model M)~\cite{ffcc}& 2017 & 1.78 & 0.96 & 1.14 & 0.29 & 4.62  & 1.99 & 1.31 & 1.43 & \textbf{0.35} & 4.75 & 8.2K \\
    \rowcolor{lightgray!30} Convolutinal-Mean~\cite{cm}& 2019 & 2.48 & 1.61 & 1.80 & 0.47 & 5.97 & 2.25 & 1.59 & 1.74 & 0.50 & 5.13 & 1.1K \\

    % \rowcolor{lightgray!30} MDLCC~\cite{mdlcc}& 2020 & 1.58 & 0.95 & 1.11 & 0.37 & 3.77 & 1.78 & 1.29 & 1.40 & 0.42 & 3.97 & 1.7M \\
    \rowcolor{lightgray!30} Multi-Hyp.~\cite{multi-hyp} & 2020 & 2.35 & 1.43 & 1.63 & 0.40 & 5.80 & 2.39 & 1.61 & 1.74 & 0.50 & 5.67 & 22.8K \\
    \rowcolor{lightgray!30} Deep Metric Learning~\cite{end2end}& 2020 & 1.58 & 0.92 & - & 0.28 & 3.70 & 1.85 & 1.24 & - & 0.36 & 4.58 & $>$4.3M \\
    \rowcolor{lightgray!30} C4~\cite{yu2020c4} & 2020 & 1.35 & 0.88 & 0.99 & 0.28 & 3.21  & 1.96 & 1.42 & 1.53 & 0.48 & 4.40 & 5.1M \\ 
    % Proposed &  2020 &  \textbf{1.27} & \textbf{0.81} & \textbf{0.90} & \textbf{0.28} & \textbf{3.04 } &  \textbf{1.72}& \textbf{1.23} & \textbf{1.32} & 0.39 & \textbf{3.87} & 0.8M \\\hline
    %  Proposed &  2020 &  \textbf{1.28} & \textbf{0.81} & \textbf{0.91} & \textbf{0.24} & \textbf{3.16 } &  \textbf{1.72}& \textbf{1.23} & \textbf{1.32} & 0.39 & \textbf{3.87} & 0.8M \\\hline
    % Proposed &  2020 &  \textbf{1.28} & \textbf{0.81} & \textbf{0.91} & \textbf{0.24} & \textbf{3.16 } &  \textbf{1.70}& \textbf{1.24} & \textbf{1.33} & 0.42 & \textbf{3.78} & 0.8M \\
    % Proposed~(pre-trained) &  2021 &  \textbf{1.27} & \textbf{0.80} & \textbf{0.90} & \textbf{0.24} & \textbf{3.13} &  \textbf{1.68}& \textbf{1.22} & \textbf{1.31} & 0.41 & \textbf{3.73} & 0.8M \\ 
    % Ours~(Pretrain w/o SAP) & 2021 & 3.25 & 2.46 & 2.52 & 0.92 & 7.13 &  2.71 & 2.02 & 2.14 & 0.79 & 5.84 & 0.8M \\ 
   
    % \rowcolor{lightgray!30} Ours~(from scratch) & 2021  &  1.27 & 0.80 & 0.90 & 0.24 & 3.13 & 1.68 & 1.22 & 1.31 & 0.41 & 3.73 & 0.8M \\
    \rowcolor{lightgray!30} Ours~(single-sensor) & 2021  &  \textbf{1.27} & \textbf{0.80} & \textbf{0.90} & \textbf{0.24} & \textbf{3.13} & \textbf{1.72} & \textbf{1.23} & \textbf{1.32} & 0.39 & \textbf{3.87} & 0.8M \\
    % \rowcolor{lightgray!30} Ours~(fine-tuned) & 2021 &  \textbf{-} & \textbf{-} & \textbf{-} & \textbf{-} & \textbf{-} & \textbf{1.64} & \textbf{-} & \textbf{-} & - & \textbf{-} & 0.8M \\
    
    \bottomrule
    \end{tabular}

    \label{tab:compare}
\end{table*}
We conduct extensive experiments on many popular datasets. We start by introducing the basics of the datasets we used and the corresponding experimental settings  in Sec.~\ref{sec:setting}. Then, we demonstrate the comparisons with state-of-the-art methods quantitatively and qualitatively in Sec.~\ref{sec:exp_compare}. Next, the evaluation of the proposed self-supervised cross-sensor training and the single-sensor sensor-aware illuminant enhancement are performed in Sec.~\ref{sec:exp_cross} and Sec.~\ref{sec:exp_single}, respectively. Finally, we provide detailed ablation study of our proposed network structure in Sec.~\ref{sec:exp_net}.

\subsection{Settings}
\label{sec:setting}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\columnwidth]{IEEEtran/figures/fig_canon5d.png}
    \caption{The illuminant distributions in $[\frac{G}{B},\frac{G}{R}]$ of \textit{Canon 5D}~(Gehler-Shi) and \textit{Canon 5DSR}~(INTEL-TAU). Obviously, the two distributions are different.}
    \label{fig:evidence}
\end{figure}

\textbf{Datasets.}
Our method is evaluated on several popular datasets, including the reprocessed Gehler-Shi dataset \cite{gehler2008bayesian,shi2000re}, the NUS 8-Camera dataset~\cite{nus8}~(NUS8), the Cube/Cube+ dataset~\cite{cube} and the Cube+ ISPA 2019 challenge dataset~\cite{cubechallenge}~(Cube-Challenge). 
Specifically, the Gehler-Shi dataset contains 568 images including indoor and outdoor scenes captured by \textit{Canon 1D}~(86 images) and \textit{Canon 5D}~(482 images) cameras. The NUS8 dataset consists of 1736 images from 8 cameras, about 210 images per camera, and each scene may be photographed by multiple cameras. The Cube+ dataset extends the original 1365 images in the Cube dataset with additional 342 images captured in nighttime outdoor and indoor scenes. And Cube-Challenge includes only 363 images for testing a network trained on Cube+. All images in Cube/Cube+/Cube-Challenge are captured by a \textit{Canon 550D} camera. 
% As for Cube-Challenge, we train the model using the Cube+ dataset~(Cube~\cite{cube} with additional 342 images captured in nighttime outdoor and indoor scenes) and test it on the 363 test images from this challenge as previously. All images in Cube/Cube+/Cube-Challenge are captured by a \textit{Canon 550D} camera.
%The Cube+ dataset extends the original 1365 images in Cube~\cite{cube} with additional 342 images captured in nighttime outdoor and indoor scenes. The Cube-Challenge dataset has only 363 images for testing the network, which is trained on Cube+.
For all images in above datasets, a Macbeth Color Checker or a SpyderCube calibration object is put in the scene to obtain the ground-truth illuminant. To avoid the influence of the calibration objects, they are masked out during both training and testing. Black-level subtraction and saturate-pixel clipping are applied after the masking out~\cite{hu2017fc4,multi-hyp}. As for UIP, we use the split of train2017 from COCO~\cite{coco} to train our network. COCO contains 330K common images, which are considered as white-balanced in our experiments. As for SAF, we use the largest available CC dataset INTEL-TAU~\cite{laakom2019intel}. INTEL-TAU contains over 7000 images which are captured by three sensors, \textit{Canon 5DSR}, \textit{Nikon D810}, and \textit{Sony IMX135}. Notice that, all the camera sensors are not overlapping for our cross-sensor evaluation. Specifically, the Canon 5D~(Gehler-Shi) is different from the Canon 5DSR~(INTEL-TAU) and we give the evidence of their different illuminant distributions in Figure~\ref{fig:evidence}.

\textbf{Data Augmentation and Pre-processing.} When training, we apply some basic data augmentation methods similar to previous works~\cite{hu2017fc4,yu2020c4,mdlcc}. 
In detail, for each training sample, we randomly crop a square patch from the original image with a side length of 0.1--1 times of the shorter dimension of the image. Then, this patch is rotated by a random angle in $[-30^{\circ}, 30^{\circ}]$, and flipped horizontally with the probability of 0.5.
Finally, we get the largest rectangle within the rotated patch and resize it into $512\times512$ resolution for training. 
In testing, we only resize the original images to 50\% of their original resolution for speed-accuracy trade-off like ~\cite{hu2017fc4,yu2020c4}. 
All the samples are pre-processed using a gamma correction factor~($\gamma=\frac{1}{2.2}$) to match the distribution of the ImageNet data that are used to pre-train the backbone. 


\textbf{Implementation Details.} We implement our network using PyTorch~\cite{paszke2019pytorch}. It is trained in an end-to-end fashion on an Nvidia Tesla V100 GPU. We train it for 4k epochs~(1k epochs for Cube-Challenge) with a batch size of 16 by the Adam optimizer~\cite{kingma2014adam} with a learning rate $3\times10^{-4}$~(divided by 2 after 2k epochs). We use the same number of stages~($M=3$) as C4. As for inference time, our model runs in real-time~(36 fps on $512\times512$ images) and shows a similar speed to the baseline C4 under the same platform. 
%Following the previous work, we load pre-trained model SqueezeNet~\cite{squeezenet} v1.1 on ImageNet~\cite{deng2009imagenet} to initial our backbone. Since our color constancy task is quite different with the image classfication task, in order to extract more helpful color features and semantic features, all the layers are trained using the ADAM~\cite{kingma2014adam} optimizer with same initial learning rate 3 $\times$ 10$^{-4}$, devided by 2 after 2000 epochs. And dropout~\cite{dropout}is also employed before the Non-Local modules to avoid over-fitting.

% Following previous works~\cite{hu2017fc4,multi-hyp,yu2020c4}, we perform three-fold cross validation for both the Gehler-Shi and NUS dataset. However the Cube+ and Cube+ challenge don't provide splits. Considering that images in both the Cube+ and Cube+ challenge dataset are collected with the same camera, so we use the Cube+ dataset as training data while the Cube+ challenge dataset serves as testing data.
%However the Cube+ and Cube+ challenge don't provide splits. Considering that images in both the Cube+ and Cube+ challenge dataset are collected with the same camera, so we use the Cube+ dataset as training data while the Cube+ challenge dataset serves as testing data. 


\textbf{Evaluation.} For fair comparison, we perform three-fold cross validations on both the Gehler-Shi and NUS datasets using the same splits as \cite{hu2017fc4,multi-hyp,yu2020c4}. When evaluating on Cube-Challenge, we use Cube+ as the training dataset and test on Cube-Challenge following the challenge guideline~\cite{cubechallenge}. Similar to previous works~\cite{yu2020c4,hu2017fc4,mdlcc}, we use the angular error $\epsilon = \frac{180}{\pi}\arccos({\frac{\ell \cdot \ell'}{\parallel \ell\parallel \parallel \ell' \parallel}})$ to measure the difference between the ground-truth illumination $\ell$ and the estimated illumination $\ell'$. We report five common CC statistics about angular errors, \ie, Mean, median~(Med.), tri-mean~(Tri.) of the errors, mean of the smallest 25\% of the errors~(Best 25\%) and mean of the largest 25\% of the errors~(Worst 25\%). The units of these metrics are degrees.




\begin{figure*}[t]
\centering
\begin{subfigure}{\xxwidth\textwidth}
    \centering
    \includegraphics[width=0.88\columnwidth]{figures/supp/canon550d2053/canon550d2053_raw.jpg}
    \vspace{-0.4em}
    \caption*{Input}
\end{subfigure}
\begin{subfigure}{\xxwidth\textwidth}
    \centering
    \includegraphics[width=\columnwidth]{figures/supp/canon550d2053/canon550d2053_fc4_pred.jpg}
    \vspace{-1.5em}
    \caption*{FC4~($4.88^{\circ}$)}
\end{subfigure}
\begin{subfigure}{\xxwidth\textwidth}
    \centering
    \includegraphics[width=\columnwidth]{figures/supp/canon550d2053/canon550d2053_c4_pred.jpg}
    \vspace{-1.5em}
    \caption*{C4~($1.05^{\circ}$)}
\end{subfigure}
\begin{subfigure}{\xxwidth\textwidth}
    \centering
    \includegraphics[width=\columnwidth]{figures/supp/canon550d2053/canon550d2053_dh_pred.jpg}
    \vspace{-1.5em}
    \caption*{Ours~($\mathbf{0.10^{\circ}}$)}
\end{subfigure}
\begin{subfigure}{\xxwidth\textwidth}
    \centering
    \includegraphics[width=\columnwidth]{figures/supp/canon550d2053/canon550d2053_gt.jpg}
    \vspace{-1.5em}
    \caption*{Ground Truth}
\end{subfigure}

% \begin{subfigure}{\xxwidth\textwidth}
%     \centering
%     \includegraphics[width=0.88\columnwidth]{figures/supp/canon550d1980/canon550d1980_raw.jpg}
%     \vspace{-0.4em}
%     \caption*{Input}
% \end{subfigure}
% \begin{subfigure}{\xxwidth\textwidth}
%     \centering
%     \includegraphics[width=\columnwidth]{figures/supp/canon550d1980/canon550d1980_fc4_pred.jpg}
%     \vspace{-1.5em}
%     \caption*{FC4~($4.06^{\circ}$)}
% \end{subfigure}
% \begin{subfigure}{\xxwidth\textwidth}
%     \centering
%     \includegraphics[width=\columnwidth]{figures/supp/canon550d1980/canon550d1980_c4_pred.jpg}
%     \vspace{-1.5em}
%     \caption*{C4~($5.93^{\circ}$)}
% \end{subfigure}
% \begin{subfigure}{\xxwidth\textwidth}
%     \centering
%     \includegraphics[width=\columnwidth]{figures/supp/canon550d1980/canon550d1980_dh_pred.jpg}
%     \vspace{-1.5em}
%     \caption*{Ours~($\mathbf{0.67^{\circ}}$)}
% \end{subfigure}
% \begin{subfigure}{\xxwidth\textwidth}
%     \centering
%     \includegraphics[width=\columnwidth]{figures/supp/canon550d1980/canon550d1980_gt.jpg}
%     \vspace{-1.5em}
%     \caption*{Ground Truth}
% \end{subfigure}

\begin{subfigure}{\xxwidth\textwidth}
    \centering
    \includegraphics[width=0.88\columnwidth]{figures/supp/canon550d2016/canon550d2016_raw.jpg}
    \vspace{-0.4em}
    \caption*{Input}
\end{subfigure}
\begin{subfigure}{\xxwidth\textwidth}
    \centering
    \includegraphics[width=\columnwidth]{figures/supp/canon550d2016/canon550d2016_fc4_pred.jpg}
    \vspace{-1.5em}
    \caption*{FC4~($3.58^{\circ}$)}
\end{subfigure}
\begin{subfigure}{\xxwidth\textwidth}
    \centering
    \includegraphics[width=\columnwidth]{figures/supp/canon550d2016/canon550d2016_c4_pred.jpg}
    \vspace{-1.5em}
    \caption*{C4~($1.92^{\circ}$)}
\end{subfigure}
\begin{subfigure}{\xxwidth\textwidth}
    \centering
    \includegraphics[width=\columnwidth]{figures/supp/canon550d2016/canon550d2016_dh_pred.jpg}
    \vspace{-1.5em}
    \caption*{Ours~($\mathbf{0.35^{\circ}}$)}
\end{subfigure}
\begin{subfigure}{\xxwidth\textwidth}
    \centering
    \includegraphics[width=\columnwidth]{figures/supp/canon550d2016/canon550d2016_gt.jpg}
    \vspace{-1.5em}
    \caption*{Ground Truth}
\end{subfigure}

% \begin{subfigure}{\xxwidth\textwidth}
%     \centering
%     \includegraphics[width=0.88\columnwidth]{figures/supp/canon550d1967/canon550d1967_raw.jpg}
%     \vspace{-0.4em}
%     \caption*{Input}
% \end{subfigure}
% \begin{subfigure}{\xxwidth\textwidth}
%     \centering
%     \includegraphics[width=\columnwidth]{figures/supp/canon550d1967/canon550d1967_fc4_pred.jpg}
%     \vspace{-1.5em}
%     \caption*{FC4~($1.47^{\circ}$)}
% \end{subfigure}
% \begin{subfigure}{\xxwidth\textwidth}
%     \centering
%     \includegraphics[width=\columnwidth]{figures/supp/canon550d1967/canon550d1967_c4_pred.jpg}
%     \vspace{-1.5em}
%     \caption*{C4~($3.28^{\circ}$)}
% \end{subfigure}
% \begin{subfigure}{\xxwidth\textwidth}
%     \centering
%     \includegraphics[width=\columnwidth]{figures/supp/canon550d1967/canon550d1967_dh_pred.jpg}
%     \vspace{-1.5em}
%     \caption*{Ours~($\mathbf{0.77^{\circ}}$)}
% \end{subfigure}
% \begin{subfigure}{\xxwidth\textwidth}
%     \centering
%     \includegraphics[width=\columnwidth]{figures/supp/canon550d1967/canon550d1967_gt.jpg}
%     \vspace{-1.5em}
%     \caption*{Ground Truth}
% \end{subfigure}




\begin{subfigure}{\xxwidth\textwidth}
    \centering
    \includegraphics[width=0.88\columnwidth]{figures/supp/8D5U5564.png/input.jpg}
    \vspace{-0.5em}
    \caption*{Input}
\end{subfigure}
\begin{subfigure}{\xxwidth\textwidth}
    \centering
    \includegraphics[width=\columnwidth]{figures/supp/8D5U5564.png/fc4_pred.jpg}
    \vspace{-1.5em}
    \caption*{FC4~($2.77^{\circ}$)}
\end{subfigure}
\begin{subfigure}{\xxwidth\textwidth}
    \centering
    \includegraphics[width=\columnwidth]{figures/supp/8D5U5564.png/c4_pred.jpg}
    \vspace{-1.5em}
    \caption*{C4~($1.32^{\circ}$)}
\end{subfigure}
\begin{subfigure}{\xxwidth\textwidth}
    \centering
    \includegraphics[width=\columnwidth]{figures/supp/8D5U5564.png/dh_pred.jpg}
    \vspace{-1.5em}
    \caption*{Ours~($\mathbf{0.67^{\circ}}$)}
\end{subfigure}
\begin{subfigure}{\xxwidth\textwidth}
    \centering
    \includegraphics[width=\columnwidth]{figures/supp/8D5U5564.png/gt.jpg}
    \vspace{-1.5em}
    \caption*{Ground Truth}
\end{subfigure}

% \begin{subfigure}{\xxwidth\textwidth}
%     \centering
%     \includegraphics[width=0.88\columnwidth]{figures/supp/IMG_0344.png/input.jpg}
%     \vspace{-0.5em}
%     \caption*{Input}
% \end{subfigure}
% \begin{subfigure}{\xxwidth\textwidth}
%     \centering
%     \includegraphics[width=\columnwidth]{figures/supp/IMG_0344.png/fc4_pred.jpg}
%     \vspace{-1.5em}
%     \caption*{FC4~($2.53^{\circ}$)}
% \end{subfigure}
% \begin{subfigure}{\xxwidth\textwidth}
%     \centering
%     \includegraphics[width=\columnwidth]{figures/supp/IMG_0344.png/c4_pred.jpg}
%     \vspace{-1.5em}
%     \caption*{C4~($1.41^{\circ}$)}
% \end{subfigure}
% \begin{subfigure}{\xxwidth\textwidth}
%     \centering
%     \includegraphics[width=\columnwidth]{figures/supp/IMG_0344.png/dh_pred.jpg}
%     \vspace{-1.5em}
%     \caption*{Ours~($\mathbf{1.16^{\circ}}$)}
% \end{subfigure}
% \begin{subfigure}{\xxwidth\textwidth}
%     \centering
%     \includegraphics[width=\columnwidth]{figures/supp/IMG_0344.png/gt.jpg}
%     \vspace{-1.5em}
%     \caption*{Ground Truth}
% \end{subfigure}

\begin{subfigure}{\xxwidth\textwidth}
    \centering
    \includegraphics[width=0.88\columnwidth]{figures/supp/IMG_0451.png/input.jpg}
    \vspace{-0.5em}
    \caption*{Input}
\end{subfigure}
\begin{subfigure}{\xxwidth\textwidth}
    \centering
    \includegraphics[width=\columnwidth]{figures/supp/IMG_0451.png/fc4_pred.jpg}
    \vspace{-1.5em}
    \caption*{FC4~($2.17^{\circ}$)}
\end{subfigure}
\begin{subfigure}{\xxwidth\textwidth}
    \centering
    \includegraphics[width=\columnwidth]{figures/supp/IMG_0451.png/c4_pred.jpg}
    \vspace{-1.5em}
    \caption*{C4~($0.91^{\circ}$)}
\end{subfigure}
\begin{subfigure}{\xxwidth\textwidth}
    \centering
    \includegraphics[width=\columnwidth]{figures/supp/IMG_0451.png/dh_pred.jpg}
    \vspace{-1.5em}
    \caption*{Ours~($\mathbf{0.42^{\circ}}$)}
\end{subfigure}
\begin{subfigure}{\xxwidth\textwidth}
    \centering
    \includegraphics[width=\columnwidth]{figures/supp/IMG_0451.png/gt.jpg}
    \vspace{-1.5em}
    \caption*{Ground Truth}
\end{subfigure}

% \begin{subfigure}{\xxwidth\textwidth}
%     \centering
%     \includegraphics[width=0.88\columnwidth]{figures/supp/IMG_0801.png/input.jpg}
%     \vspace{-0.5em}
%     \caption*{Input}
% \end{subfigure}
% \begin{subfigure}{\xxwidth\textwidth}
%     \centering
%     \includegraphics[width=\columnwidth]{figures/supp/IMG_0801.png/fc4_pred.jpg}
%     \vspace{-1.5em}
%     \caption*{FC4~($0.55^{\circ}$)}
% \end{subfigure}
% \begin{subfigure}{\xxwidth\textwidth}
%     \centering
%     \includegraphics[width=\columnwidth]{figures/supp/IMG_0801.png/c4_pred.jpg}
%     \vspace{-1.5em}
%     \caption*{C4~($0.13^{\circ}$)}
% \end{subfigure}
% \begin{subfigure}{\xxwidth\textwidth}
%     \centering
%     \includegraphics[width=\columnwidth]{figures/supp/IMG_0801.png/dh_pred.jpg}
%     \vspace{-1.5em}
%     \caption*{Ours~($\mathbf{0.08^{\circ}}$)}
% \end{subfigure}
% \begin{subfigure}{\xxwidth\textwidth}
%     \centering
%     \includegraphics[width=\columnwidth]{figures/supp/IMG_0801.png/gt.jpg}
%     \vspace{-1.5em}
%     \caption*{Ground Truth}
% \end{subfigure}

\caption{Comparisons among the proposed method, C4~\cite{yu2020c4} and FC4~\cite{hu2017fc4}. For each method, we visualize the corrected image on the left of each predicted illuminant, and report the angular error compared with the corresponding ground truth below each image. The upper two images are taken from Cube-Challenge while the other two are from Gehler-Shi. Note that the calibration objects are masked out when training and testing.}
\label{fig:visual}
\end{figure*}


\begin{table}[t]
    \small 
    \centering
    \caption{Comparison with the state-of-the-art methods on the Cube-Challenge dataset. The \colorbox{lightgray!30}{shadowed} methods are for single-sensor evaluation while the others are for  cross-sensor evaluation.}

    \begin{tabular}{l|ccccc}
    \toprule
    Method &  Mean & Med. & Tri. & Best & Worst \\
     &   &  &  & 25\% & 25\% \\\hline
    Grey World~\cite{gray-world} & 4.44 & 3.50 & - & 0.77 & 9.64 \\
    1st Gray-Edge~\cite{gray-edge}& 3.51 & 2.30 & - & 0.56 & 8.53 \\
    V Vuk \etal~\cite{cubechallenge}& 6.00 & 1.96 & 2.25 & 0.99 & 18.81 \\
    SIIE~\cite{siie}&  2.10 & 1.23 & - & 0.47 & 5.38 \\
    Multi-Hyp.~\cite{multi-hyp} & 1.99 & \textbf{1.06} & \textbf{1.14} & \textbf{0.35} & 5.35 \\
    Ours~(cross-sensor) & \textbf{1.75} & 1.26 & 1.32 & 0.42 & \textbf{4.04} \\ \hline
    \rowcolor{lightgray!30} Y Qian \etal~\cite{cubechallenge}& 2.21 & 1.32 & 1.41 & 0.43 & 5.65 \\
    \rowcolor{lightgray!30} K Chen \etal~\cite{cubechallenge}& 1.84 & 1.27 & 1.32 & 0.39 & 4.41 \\
    \rowcolor{lightgray!30} FFCC~(model J)~\cite{ffcc}& 2.10 & 1.23 & 1.34 & 0.47 & 5.38 \\
    \rowcolor{lightgray!30} A Savchik \etal~\cite{cubechallenge}& 2.05 & 1.20 & 1.30 & 0.40 & 5.24 \\
    \rowcolor{lightgray!30} WB-sRGB~\cite{afifi2019color}& 1.83 & 1.15 & - & 0.35 & 4.60 \\
    \rowcolor{lightgray!30} FC4~\cite{hu2017fc4}  &  1.75 & 1.00 & 1.13 & 0.37 & 4.45\\
    \rowcolor{lightgray!30} C4~\cite{yu2020c4}  & 1.76 & 1.11 & 1.25 &  0.37 &   4.54  \\
    % \hline
    %Mean: 1.750803, Med: 1.258966, tri: 1.317533, bst: 0.418255, wst: 4.044954, pct: 5.335168

    %  Ours~(Pre-trained) & \textbf{1.90} & 1.54 & 1.60 &  0.55 & \textbf{3.92}  \\
    \rowcolor{lightgray!30} Ours~(single-sensor) & 1.57 & \textbf{0.91} & 1.06 & 0.31 & 3.92  \\
    % \rowcolor{lightgray!30} Ours~(fintune) & \textbf{1.49} & 0.99 & \textbf{1.06} & \textbf{0.31} & \textbf{3.56}  \\
    \rowcolor{lightgray!30} Ours~(fine-tuning) & \textbf{1.47} & 0.95 & \textbf{1.02} & \textbf{0.30} & \textbf{3.60}  \\
    \bottomrule
    \end{tabular}
    \label{tab:cubec}
\end{table}

% \begin{figure*}[t!]
%     \centering
%     \begin{subfigure}[t]{0.245\textwidth}
%         \centering
%         \includegraphics[width=\columnwidth]{figures/fewshot.png}
%         \vspace{-2em}
%         \caption{Mean}
%         \label{fig:relighting_a}
%     \end{subfigure}%
%     \begin{subfigure}[t]{0.245\textwidth}
%         \centering
%         \includegraphics[width=\columnwidth]{figures/best25.png}
%         \vspace{-2em}
%         \caption{Best 25\%}
%         \label{fig:relighting_b}
%     \end{subfigure}
%     \begin{subfigure}[t]{0.245\textwidth}
%         \centering
%         \includegraphics[width=\columnwidth]{figures/wst25.png}
%         \vspace{-2em}
%         \caption{Worst 25\%}
%         \label{fig:relighting_c}
%     \end{subfigure}
%     \begin{subfigure}[t]{0.245\textwidth}
%         \centering
%         \includegraphics[width=\columnwidth]{figures/his.png}
%         \vspace{-2em}
%         \caption{Histogram of angular errors}
%         \label{fig:relighting_d}
%     \end{subfigure}
%     \vspace{-1em}
%     \caption{Effect of different relighting methods with the growth of training samples. (a)~Mean angular error. (b)~Mean of the Best 25\%. (c)~Mean of the Worst 25\%. (d)~Normalized histogram of angular errors when $K=100$ to show the robustness of our relighting method in the long-tailed data distribution.}
%     \label{fig:relighting}
% \end{figure*}


% \begin{figure*}[t!]
%     \centering
%     \begin{subfigure}[t]{0.245\textwidth}
%         \centering
%         \includegraphics[width=\columnwidth]{figures/cubec_fewshot.png}
%         \vspace{-2em}
%         \caption{Mean}
%         \label{fig:relighting_a}
%     \end{subfigure}%
%     \begin{subfigure}[t]{0.245\textwidth}
%         \centering
%         \includegraphics[width=\columnwidth]{figures/cubec_best25.png}
%         \vspace{-2em}
%         \caption{Best 25\%}
%         \label{fig:relighting_b}
%     \end{subfigure}
%     \begin{subfigure}[t]{0.245\textwidth}
%         \centering
%         \includegraphics[width=\columnwidth]{figures/cubec_wst25.png}
%         \vspace{-2em}
%         \caption{Worst 25\%}
%         \label{fig:relighting_c}
%     \end{subfigure}
%     \begin{subfigure}[t]{0.245\textwidth}
%         \centering
%         \includegraphics[width=\columnwidth]{figures/cubec_training.png}
%         \vspace{-2em}
%         \caption{Training process}
%         \label{fig:relighting_d}
%     \end{subfigure}
%     \vspace{-1em}
%     \caption{Effect of different relighting methods with the growth of training samples. (a)~Mean angular error. (b)~Mean of the Best 25\%. (c)~Mean of the Worst 25\%. (d)~Training process on the full Cube-Challenge dataset.}
%     \vspace{-1em}
%     \label{fig:relighting}
% \end{figure*}

\subsection{Comparison with State-of-the-Art Methods}
\label{sec:exp_compare}
We compare our method with a number of representative algorithms, including widely-used statistics-based~\cite{white-patch,gray-world,gray-edge,shades-of-gray}, early machine learning-based~\cite{SVR,gehler2008bayesian} and recent deep learning-based~\cite{bianco2015color,cm,ccc,ffcc,hu2017fc4,yu2020c4,siie,end2end}.

The numeric results on the widely-used  Gehler-Shi, NUS8 and Cube-Challenge datasets are reported in Tables~\ref{tab:compare} and~\ref{tab:cubec}. All our experiments are trained on the proposed network. In the cross-sensor setting, we train the network on COCO~\cite{coco} and INTEL-TAU~\cite{laakom2019intel} with the proposed  self-supervised cross-sensor training method and evaluate its performance. In the single-sensor experiments, without UIP and SAF, we train our network from scratch using the sensor-aware illuminant enhancement~(SIE) described in Section~\ref{sec32}.

%in terms of the Mean, Median, Tri-mean, the Best 25\% and the Worst 25\% of the angular errors. 
%We report the performance of the settings on cross-sensor evaluation with \textit{a single trained model}~(Pretrain w/ UP \& SAP), the single-sensor model using the corresponding sensor data along~(from scratch) and the model finetuned on the proposed pre-trained model~(fine-tuned) on these benchmarks. 
As for the cross-sensor evaluation, although our model is fully trained with the synthesized illuminants, it still obtains significantly better performance than other cross-sensor methods by a large margin. On the carefully collected single-sensor evaluation datasets~(NUS8 and Cube-Challenge), our cross-sensor model even performs better than most of single-sensor models owing to the proposed UIP and SAF. Also, we argue that compared with previous cross-sensor methods, training with UIP and SAF can gain much more \textit{robust} results in terms of the metric of Worst 25\%. 

%Specifically, the proposed method show much better results on two dataset than out baselines~(C4~\cite{yu2020c4}, FC4~\cite{hu2017fc4}). 
On the other hand, the proposed network structure is also the key to achieve the state-of-the-art performance. We evaluate the performance of the proposed network trained \textit{from scratch} and it shows a much better performance than other methods in Tables~\ref{tab:compare} and~\ref{tab:cubec}~(see the single-sensor comparison). Finally, as shown in the last row of Table~\ref{tab:cubec}, by fine-tuning the cross-sensor model on the specific sensor, the performance can be further boosted. 

%the network~({\color{red}about 17\% better~(Mean) than the baseline C4~\cite{yu2020c4} and 10\% better than the previous most accurate method~\cite{end2end}}). 

In addition to the numerical comparisons, we also show some visual comparisons on Gehler-Shi and Cube-Challenge with FC4 and C4. To get the visual results, we directly use the trained models from the Github page\footnote{\url{https://github.com/yhlscut/C4}.} on the Gehler-Shi dataset, and train them from scratch on Cube-Challenge with the default settings. As shown in Figure~\ref{fig:visual}, our method shows a significant advantage over the two baselines. We also find our model is very good at handling the situation when the scenes contain few objects~(top two samples in Figure~\ref{fig:visual}), which might be because the proposed sensor-aware illuminant enhancement is based on the von Kries assumption and these scenes are more consistent with this assumption.  

\begin{table*}[!t]
    \centering
    \caption{The mean of angular errors on \textit{cross-sensor} evaluation which directly evaluates pre-trained methods on various sensors without single-sensor fine-tuning. Both the methods Naive and SAF use the INTEL-TAU dataset~\cite{laakom2019intel} for training, while UIP uses COCO~\cite{coco}. Notice that the sensors from the training sets are different from those in the testing sets (Gehler-Shi, NUS8 and Cube-Challenge). The {\color{blue}blue} and {\color{red}red} numbers are the relative {\color{blue}improvement} and {\color{red}decline}, compared with the model trained by Naive method. All the methods are based on the proposed network.} %The first 8 sensors and \textit{Canon 550D} are from NUS8 and Cube-Challenge, respectively.}
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{l|llllllll|l|l}
    \toprule
    Datasets & \multicolumn{8}{c|}{NUS8} & Cube-Challenge & \multicolumn{1}{c}{Gehler-Shi} \\ \hline
    Method & \textit{Canon 1D} & \textit{Canon 600D} & \textit{Fuji} & \textit{Nikon 52} & \textit{Olympus} & \textit{Panasonic} & \textit{Samsung} & \textit{Sony} & \textit{Canon 550D} & \textit{Canon 5D\&1D} \\ \hline
     Naive &3.07 &2.61 &3.66 &3.45 &3.25 &2.41 &2.92 &3.49 &2.76 & 3.71\\
     SAF &2.09~({\color{blue}{\footnotesize0.98}})
     &2.07~({\color{blue}{\footnotesize0.54}})
     &2.15~({\color{blue}{\footnotesize1.51}})
     &2.14~({\color{blue}{\footnotesize1.31}})
     &\textbf{1.88}~({\color{blue}{\footnotesize1.37}})
     &2.13~({\color{blue}{\footnotesize0.28}})
     &2.05~({\color{blue}{\footnotesize0.87}})
     &1.95~({\color{blue}{\footnotesize1.54}})
     &1.91~({\color{blue}{\footnotesize0.85}})
     &2.58~({\color{blue}{\footnotesize1.13}})\\
     UIP &6.82~({\color{red}{\footnotesize3.75}})
     &9.24~({\color{red}{\footnotesize6.63}})
     &8.12~({\color{red}{\footnotesize4.46}})
     &9.48~({\color{red}{\footnotesize6.03}})
     &9.07~({\color{red}{\footnotesize5.82}})
     &10.44~({\color{red}{\footnotesize8.03}})
     &11.59~({\color{red}{\footnotesize8.67}})
     &7.51~({\color{red}{\footnotesize4.02}})
     &5.53~({\color{red}{\footnotesize2.77}})
     &7.27~({\color{red}{\footnotesize3.56}})\\
    UIP\&SAF &\textbf{1.99}~({\color{blue}{\footnotesize1.08}})
    &\textbf{1.80}~({\color{blue}{\footnotesize0.81}})
    &\textbf{2.12}~({\color{blue}{\footnotesize1.54}})
    &\textbf{2.11}~({\color{blue}{\footnotesize1.34}})
    &1.93~({\color{blue}{\footnotesize1.32}})
    &\textbf{1.94}~({\color{blue}{\footnotesize0.47}})
    &\textbf{2.04}~({\color{blue}{\footnotesize0.88}})
    &\textbf{1.90}~({\color{blue}{\footnotesize1.59}})
    &\textbf{1.75}~({\color{blue}{\footnotesize1.01}})
    & \textbf{2.46}~({\color{blue}{\footnotesize1.25}}) \\
    \bottomrule
    \end{tabular}}
    \label{tab:xcc}
\end{table*}


\begin{table*}[!t]
    \centering
    \small
    \caption{The mean of angular errors on \textit{single-sensor} fine-tuning evaluation using different pre-trained cross-sensor methods on 8 NUS8 subsets and Cube-Challenge~(\textit{Canon 550D}). The {\color{blue}blue} and {\color{red}red} numbers are the relative {\color{blue}improvement} and {\color{red}decline}, compared with the model trained from scratch. All the methods are based on the proposed network.}
    \begin{tabular}{l|lllllllll}
    \toprule
    Method & \textit{Canon 1D} & \textit{Canon 600D} & \textit{Fuji} & \textit{Nikon 52} & \textit{Olympus} & \textit{Panasonic} & \textit{Samsung} & \textit{Sony} & \textit{Canon 550D} \\ \hline
    Scratch &1.84 &1.67 &1.86 &1.85 &\textbf{1.43} &1.77 &1.78 &1.59 &1.57\\
    Naive &1.77~({\color{blue}{\footnotesize0.07}}) &1.67~({\color{black}{\footnotesize0.0}}) &1.79~({\color{blue}{\footnotesize0.07}}) & 1.77~({\color{blue}{\footnotesize0.08}}) & 1.57~({\color{red}{\footnotesize0.14}}) &1.77~({\color{black}{\footnotesize0.0}}) &1.78~({\color{black}{\footnotesize0.0}}) &1.64~({\color{red}{\footnotesize0.05}}) &1.57~({\color{black}{\footnotesize0.0}})\\
    SAF &\textbf{1.74}~({\color{blue}{\footnotesize0.10}}) &1.62~({\color{blue}{\footnotesize0.05}}) &1.71~({\color{blue}{\footnotesize0.15}}) &1.84~({\color{blue}{\footnotesize0.01}}) &1.53~({\color{red}{\footnotesize0.10}}) &1.71~({\color{blue}{\footnotesize0.06}}) & 1.79~({\color{red}{\footnotesize0.01}}) &1.56~({\color{blue}{\footnotesize0.03}}) &1.51~({\color{blue}{\footnotesize0.06}})\\
    UIP &1.77~({\color{blue}{\footnotesize0.07}}) &\textbf{1.52}~({\color{blue}{\footnotesize0.15}}) &\textbf{1.68}~({\color{blue}{\footnotesize0.18}}) &1.82~({\color{blue}{\footnotesize0.03}}) &1.46~({\color{red}{\footnotesize0.03}}) &\textbf{1.60}~({\color{blue}{\footnotesize0.17}}) &1.77~({\color{blue}{\footnotesize0.01}}) &\textbf{1.54}~({\color{blue}{\footnotesize0.05}}) &1.49~({\color{blue}{\footnotesize0.08}})\\
    UIP\&SAF &1.78~({\color{blue}{\footnotesize0.06}}) & 1.58~({\color{blue}{\footnotesize0.09}}) &1.70~({\color{blue}{\footnotesize0.16}}) &\textbf{1.74}~({\color{blue}{\footnotesize0.11}}) &1.48~({\color{red}{\footnotesize0.05}}) &1.61~({\color{blue}{\footnotesize0.16}}) &\textbf{1.72}~({\color{blue}{\footnotesize0.06}}) &1.56~({\color{blue}{\footnotesize0.03}}) &\textbf{1.47}~({\color{blue}{\footnotesize0.10}})\\
    \bottomrule
    \end{tabular}
    \label{tab:finetune}
\end{table*}


\begin{figure*}[t!]
    \centering
    \begin{subfigure}[t]{0.8\columnwidth}
        \centering
        \includegraphics[width=\columnwidth]{IEEEtran/figures/fig_norelighting.png}
        \vspace{-1em}
        \caption{Naive}
        \label{fig:cda}
    \end{subfigure}%
    \begin{subfigure}[t]{0.8\columnwidth}
        \centering
        \includegraphics[width=\columnwidth]{IEEEtran/figures/fig_relighting.png}
        \vspace{-1em}
        \caption{SAF}
        \label{fig:cdb}
    \end{subfigure}
    \caption{The effect of SAF in cross-sensor training. (a)~The distribution of illuminants in the $[\frac{G}{B},\frac{G}{R}]$ color space, which are predicted by our network trained on INTEL-TAU and tested on Gehler-Shi~\cite{gehler2008bayesian,shi2000re}. (b)~The proposed SAF trains the network with randomly generated illuminants, which successfully fits the evaluation sensor's domain. }
    \label{fig:cd}
\end{figure*}

As for the model size, the proposed network uses only 17\% of the parameters of C4 and 47\% of FC4, which further shows the advantage and the potential of our method applying on embedded devices, such as mobile phones and digital cameras. 



\subsection{Evaluation of Self-Supervised Cross-Sensor Training}
\label{sec:exp_cross}
Firstly, we evaluate the effect of the proposed unprocessing sRGB Images for Pre-Training~(UIP) and Sensor Alignment Fine-Tuning~(SAF) on three unseen datasets~(Gehler-Shi, NUS8 and Cube-Challenge) as shown in Table~\ref{tab:xcc}. We can see that although SAF without UIP trains the network with fully synthesized random illuminants, it obtains better results than training with only real illuminants~(Naive). We show an example in Figure~\ref{fig:cd} to compare the performance of the network using Naive and SAF. The network using Naive predicts a wrong color distribution for the target sensor~(a), while the network using SAF can fit the target distribution well~(b). These results show the advantage of training on the aligned domain using random illuminants. 



% \begin{table}[t]
%     \small 
%     \centering
%     \caption{The effect of cross-sensor training. Both the methods Naive and SAF use the INTEL-TAU dataset~\cite{laakom2019intel} for training, while UIP uses COCO~\cite{coco}. Notice that the sensors from the training sets are different from those in the testing sets~(Gehler-Shi, NUS8 and Cube-Challenge). All the training methods are based on our model.}
%     \begin{tabular}{l|cc|cc|cc}
%     \toprule
%     \multicolumn{1}{c|}{Training} &  \multicolumn{2}{c|}{Gehler-Shi}  & \multicolumn{2}{c|}{NUS8} & \multicolumn{2}{c}{Cube-Challenge} \\\cline{2-7}
%     \multicolumn{1}{c|}{Method} & Mean & Med. & Mean & Med. & Mean & Med. \\ \hline
%     Naive & 3.71 & 2.59 & 3.08 & 2.23 & 2.76 & 1.76 \\
%     SAF&  2.58 &  2.17 & 2.05 & 1.53 & 1.91 & 1.54 \\
%     % I-T + Cube & SAP &  \textbf{2.36} &  \textbf{1.93} & \textbf{1.96} & \textbf{1.46}  \\
%     UIP  &  7.27 &  4.66 & 8.92 & 6.82 & 5.53 & 3.18  \\
%     UIP\&SAF &  \textbf{2.46} &  \textbf{1.89} & \textbf{1.98} & \textbf{1.42} & \textbf{1.75} & \textbf{1.26} \\
   
%     \bottomrule
%     \end{tabular}
%     \label{tab:xcc}
% \end{table}



As for UIP, since the images $I_{uip}$ (unprocessed from sRGB images) are still different from real RAW images $I_{raw}$, the performance of the network using only UIP is not good enough when evaluated on the RAW images in the testing datasets. However, the advantage of UIP is that sRGB images are abundant and the network can learn the knowledge of different scenes and illuminants. We further fine-tune the network with SAF~(UIP\&SAF), it obtains the best results in Table~\ref{tab:xcc}, and outperforms other state-of-the-art cross-sensor methods as shown in Tables~\ref{tab:compare} and \ref{tab:cubec}.


We also evaluate the transferable ability of the different pre-trained cross-sensor models for single-sensor fine-tuning.
%Since it is hard to collect a large labelled dataset when there is a novel sensor, the transferable ability of the pre-trained cross-sensor model is also a concern for single-sensor fine-tuning. 
As shown in Table~\ref{tab:finetune}, the proposed unprocessing sRGB images for pre-training~(UIP), sensor alignment fine-tuning~(SAF) and UIP\&SAF training strategies can improve the performance of the single-sensor model trained from scratch. Note that when we just pre-train our network with images from multiple sensors~(Naive), the performance cannot be improved in most cases~( \textit{Canon 600D, Olympus, Panasonic, Samsung, Sony, Canon 550D} in the second row of Table~\ref{tab:finetune}).  Interestingly, although the UIP model cannot obtain satisfactory results when we evaluate it directly on specific sensors~(as shown in Table~\ref{tab:xcc}), this model has a strong transferable ability when fine-tuning it on a single sensor~(as shown in Table~\ref{tab:finetune}). It might be because the large-scale semantic information learned by UIP benefits accurate color constancy. To summarize, the UIP\&SAF method can improve the performance by a large range in most cases. 

%As shown in Table~\ref{tab:compare}, by fine-tuning the cross-domain UP model on the specific-sensors, our method show a much better performance than the model which is trained from scratch. {\color{red} Interesting, we further finetune the UP model using SAP.}


\begin{table}[t]
    \centering
     \caption{Effect of the percentage of different training combinations. The best results are bold and the second best are underlined.}
    \resizebox{\columnwidth}{!}{%
    
    \begin{tabular}{c|c|c|c|c}
    \toprule
    Dataset & Random & No Aug. & Reshuffle & Mean  \\ \hline
    \textit{Sony}    &  100\% & 0  &  0   & 1.97 \\
    \textit{Sony}    &  0  & 100\% &  0   & 1.92 \\ 
     \textit{Sony}   &  0  & 0     & 100\% & 1.80 \\
    \textit{Sony}    &  0  & 50\%  & 50\%  & \textbf{1.76} \\
    \textit{Sony}    &  33\% & 33\% & 34\% & \underline{1.79} \\ 
    \hline
    \textit{Nikon 52}   &  100\% & 0  &  0   & 2.30 \\
    \textit{Nikon 52}   &  0  & 100\% &  0   & 2.26 \\ 
    \textit{Nikon 52}   &  0  & 0     & 100\%  & \textbf{2.05} \\
    \textit{Nikon 52}    &  0  & 50\%  & 50\%  & 2.13 \\
    \textit{Nikon 52}    &  33\% & 33\% & 34\% & \underline{2.07} \\
    \bottomrule
    \end{tabular}
}
\label{tab:precentage}
\end{table}


\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\columnwidth]{figures/relighting_methods.png}
    \caption{Performances of different relighting methods on various models.}
    \label{fig:relighting_methods}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figures/relighting_dataset.png}
    \caption{Performances of different relighting methods on various datasets.}
    \label{fig:ab_more_relight}
\end{figure}


% \begin{figure*}[t]
% \hfill
% \begin{minipage}[b]{0.3\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{figures/relighting_methods.png}
%     \captionof{figure}{Performances of different relighting methods on various models.}
%     \label{fig:relighting_methods}
%   \end{minipage}
% \hfill
% \begin{minipage}[b]{0.34\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{figures/relighting_dataset.png}
%     \captionof{figure}{Performances of different relighting methods on various datasets.}
%     \label{fig:ab_more_relight}
%   \end{minipage}
% \end{figure*}

\subsection{Evaluation of Sensor-Aware Illuminant Enhancement for Single-Sensor Training}
\label{sec:exp_single}

In this section, we discuss the effect of the sensor-aware illuminant enhancement when training from \textit{scratch} for single-sensor training. 

\textbf{Percentages on Different Training Combinations.}
As discussed in Section~\ref{sec32}, we alternatively use three different types of relighting methods on the fly to train our network. Here, we evaluate the percentages of the training combinations among the three methods on the \textit{Nikon 52} and \textit{Sony} subsets of NUS8 using FC4~\cite{hu2017fc4}, as shown in Table~\ref{tab:precentage}. It is clear that using the sensor-aware label reshuffle~(Reshuffle) solely performs better than no-relighting~(No Aug.) and random relighting~(Random~\cite{hu2017fc4}). Moreover, we find that the network may get further improvement and robustness when there are multiple training combinations. Thus, in all the experiments, we equally choose samples from these three training combinations, which is a hybrid training strategy for single-sensor training.


% \begin{table}[t]

%     \centering
%     \caption{Effect of the percentage of different training combinations. The best results are bold and the second best are underlined.}
%     \begin{tabular}{c|c|c|c|c}
%     \toprule
%     Dataset & Random & No Aug. & Reshuffle & Mean  \\ \hline
%     \textit{Sony}    &  100\% & 0  &  0   & 1.97 \\
%     \textit{Sony}    &  0  & 100\% &  0   & 1.92 \\ 
%      \textit{Sony}   &  0  & 0     & 100\% & 1.80 \\
%     \textit{Sony}    &  0  & 50\%  & 50\%  & \textbf{1.76} \\
%     \textit{Sony}    &  33\% & 33\% & 34\% & \underline{1.79} \\ 
%     \hline
%     \textit{Nikon 52}   &  100\% & 0  &  0   & 2.30 \\
%     \textit{Nikon 52}   &  0  & 100\% &  0   & 2.26 \\ 
%     \textit{Nikon 52}   &  0  & 0     & 100\%  & \textbf{2.05} \\
%     \textit{Nikon 52}    &  0  & 50\%  & 50\%  & 2.13 \\
%     \textit{Nikon 52}    &  33\% & 33\% & 34\% & \underline{2.07} \\
%     % \hline
%     % \textit{Gehler-Shi}    &  100\% &  0 & 0  & 1.65 \\
%     % \textit{Gehler-Shi}    & 50\%  & 50\% &  0  & \underline{1.59} \\ 
%     % \textit{Gehler-Shi}    &  33\% & 33\% & 34\% & \textbf{1.53} \\
%     \bottomrule
%     \end{tabular}
%     \label{tab:precentage}
% \end{table}
% \begin{figure}
%     \centering
%     \includegraphics[width=0.7\columnwidth]{figures/relighting_methods.png}
%     \caption{Evaluation of scene relighting methods on different models. We show the backbone below each method.}
%     \label{fig:relighting_methods}
% \end{figure}

% \begin{figure}[t!]
%     \centering
%     \includegraphics[width=0.8\columnwidth]{figures/relighting_dataset.png}
%     \caption{Performances of different relighting methods on various datasets.}
%     \label{fig:ab_more_relight}
% \end{figure}



% \pythonFile[subfiles/]{code}

% \begin{figure}
%     \centering
%     \includegraphics[width=\columnwidth]{figures/carbon.png}
%     \caption{Simple code of the proposed relighting methods.}
%     \label{fig:my_label}
% \end{figure}


% \section{Per-Sensor evaluation on NUS8 dataset}

% \begin{figure}
%     \centering
%     \includegraphics[width=\columnwidth]{figures/training.png}
%     \caption{Validation error of different relighting methods on the Cube-Challenge using FC4~\cite{hu2017fc4}. Proposed relighting method can stabilize the training process and get better performance while no-relighting~(No Aug.) over-fit early and random relighting hurt the performance. }
%     \label{fig:overfit}
% \end{figure}



% \section{Comparison with CROP}
% \section{Relationship with recurrently neural network~(RNN)}
\textbf{Scene Relighting Methods on Different Models.}
We train different networks, including SqueezeNet-FC4~\cite{hu2017fc4}, SqueezeNet-C4~\cite{yu2020c4} and the proposed network~(with either SqueezeNet or AlexNet as the backbone), using different data augmentation methods on Cube-Challenge as shown in Figure~\ref{fig:relighting_methods}. The proposed sensor-aware illuminant enhancemant can significantly improve the performances of these networks, especially for FC4. We also note that compared with no-relighting, the random relighting also benefits C4 since C4 is very heavy~(its parameters are 6 times more than ours) and needs more training data to avoid overfitting.




% \subsection{Comparison on Scene Relighting Methods}


\textbf{Effect on Different Datasets.}
We also evaluate different scene relighting methods as data augmentation for individual and multiple sensors using FC4~\cite{hu2017fc4}. For single camera evaluation, we train FC4 and evaluate its performance on the \textit{Sony} and \textit{Nikon52} subsets of NUS8~\cite{nus8} and the \textit{Canon 5D} part of the Gehler-Shi dataset. As for multiple camera learning, the evaluations are performed on the full Gehler-Shi dataset and on the combination of the \textit{Sony} and \textit{Nikon52} subsets. As shown in Figure~\ref{fig:ab_more_relight}, The proposed hybrid training strategy obtains much better results than the previous random relighting~(Random) and no-relighting~(No~Aug.) methods on both the single and multiple camera settings. Interestingly, we find random relighting~\cite{hu2017fc4} 
only performs better on the Gehler-Shi dataset than no-relighting. It might be because Gehler-Shi contains extremely imbalanced sensor data distribution~(482~(\textit{Canon 5D})~:~86~(\textit{Canon 1D})) and the small subset~(86) provides little useful camera property guidance.
Thus, we argue that although random relighting has been widely-used in recent methods~\cite{hu2017fc4,mdlcc,yu2020c4}, it might \textit{hurt} the performance in most cases.


% \subsection{Comparison on Sensor-aware Scene Relighting Methods}

% \textbf{Effect on Different Datasets.}
% We evaluate different scene relighting methods as data augmentation for individual and multiple sensors, using one of the widely-used structures FC4~\cite{hu2017fc4}. For single camera evaluation, we train FC4 and evaluate its performance on the \textit{Sony} and \textit{Nikon52} subsets of NUS8~\cite{nus8} and the \textit{Canon 5D} part of the Gehler-Shi dataset. As for multiple camera learning, the evaluations are performed on the full Gehler-Shi dataset and on the combination of the \textit{Sony} and \textit{Nikon52} subsets. As shown in Figure~\ref{fig:ab_more_relight}, the proposed method obtains much better results than the previous random relighting~(Random) and no-relighting methods~(No~Aug.) on both the single and multiple camera settings. Interestingly, we find random relighting~\cite{hu2017fc4} 
% only performs better on the Gehler-Shi dataset than no-relighting. It might be because Gehler-Shi contains extremely imbalanced sensor data distribution~(482~(\textit{Canon 5D})~:~86~(\textit{Canon 1D})) and the small dataset~(86) provides less useful camera property guidance.
% Thus, although random relighting has been widely-used in recent methods~\cite{hu2017fc4,mdlcc,yu2020c4}, it might \textit{hurt} the performance in most cases.
% Besides the evaluation on different datasets, the proposed data augmentation method also works well on a wide range of deep models, including FC4~\cite{hu2017fc4}, C4~\cite{yu2020c4} and our network. We show more experiments in the supplementary materials.

% {\color{red}
% To evaluate the performance over different network structure, besides the FC4~\cite{hu2017fc4} and the proposed method, we also evaluate the effect of different scene relighting methods over the previous well-used color constancy method FFCC~\cite{ffcc}. As shown in the Figure~\ref{fig:srb}, the proposed scene relighting method also works well on different methods, which show the superior of the proposed methods.}





% When we use the original Random~(R) scene relighting, the angular error outperforms the methods without~(w/o) the scene relighting. Moreover, if we combine the proposed label shuffle~(S) methods and the randomly scene relighting methods, the network gain much better results. This phenomenon is not restricted to a particular network structure or sensor~(dataset). Thus, Besides Gehler-Shi dataset~\cite{shi2000re,gehler2008bayesian} as ablation study, we also evaluate the proposed data augmentation technique on the Sony and Nikon52 subset of NUS8~\cite{nus8} in Figure~\ref{fig:ab_more_relight}. The experiment results also prove the advantage of the proposed method.  


% \begin{table*}[!t]
%     \small
%     \centering
%     \caption{Ablation Study of Network Structure on Cube challenge.}
%     \vspace{-1em}
%     \begin{tabular}{l|c|c|c|ccccc}
%     \toprule
%     Model & Relighting & \# Param. & FLOPs  & Mean & Med. & Tri. & Best  & Worst  \\
%     &  &  &  &  & & & 25\% & 25\% \\\hline
%     % FC4~\cite{hu2017fc4} & Random & \underline{1.70M} & \textbf{1.59G} & 1.97 & 1.24& 1.36 & 0.46 & 4.77\\
%     FC4~\cite{hu2017fc4} (1 stage backbone of the proposed network) & w/o & \underline{1.70M} & \textbf{1.59G} & 1.87 & 1.10& 1.21 & 0.43 & 4.66\\
%     % FC4~\cite{hu2017fc4} & Proposed & \underline{1.70M} & \textbf{1.59G} & 1.61 & 0.95 & 1.01 & 0.33 & 4.14\\
%     C4~\cite{yu2020c4}(Only pre-trained backbone) & w/o & 5.11M & 4.77G & N/A & N/A & N/A & N/A & N/A  \\
%     % C4~\cite{yu2020c4}(Finetune on FC4~\cite{hu2017fc4}) & Random & 5.11M & 4.77G & 1.84 & 1.11 & 1.25 & 0.38 & 4.54  \\ 
%     C4~\cite{yu2020c4}(Finetune on FC4~\cite{hu2017fc4}) & w/o & 5.11M & 4.77G & 1.84 & 1.11 & 1.26 & 0.44 & 4.53  \\ 
%     % C4~\cite{yu2020c4}(Finetune on FC4~\cite{hu2017fc4}) & Proposed & 5.11M & 4.77G & 1.62 & 1.01 & 1.07 & 0.38 & 4.03  \\ \hline
%     Shared-C4 & w/o & 1.70M & 4.77G & 1.75 & 1.00 & 1.10 & 0.33 & 4.54 \\
%     Shared-C4 \& Share-AM & w/o & 1.75M & 4.77G & 1.84 & 1.09 & 1.20 & 0.35 & 4.67 \\
%     Shared-C4 \& ISAM~(Only last) & w/o & 1.80M & 4.77G & 1.70 & 1.04 & 1.10 & 0.34 & 4.24 \\
%     Shared-C4 \& ISAM & w/o & 1.84M & 4.77G & 1.67 & 1.04 & 1.12 & 0.33 & 4.11 \\
%     Shared-C4 \& ISAM & Random & 1.84M & 4.77G & 1.69 & 1.08 & 1.18 & 0.29 & 4.17 \\
%     % Share-C4 \& Unshare-ISAM~(Only Channel Attention) & w/o & 1.84M & 4.77G & 1.68 & 0.88 & 0.98 & 0.27 & 4.54 \\
%     Shared-C4 \& ISAM & Proposed & 1.84M & 4.77G & \underline{1.60} & \underline{0.93} & \textbf{1.01} & \textbf{0.29} & \underline{4.10} \\
%     Shared-C4 \& ISAM \& Lightweight Head & Proposed & \textbf{0.82M} & \underline{3.93G} & \textbf{1.57} & \textbf{0.91} & \underline{1.06} & \underline{0.31} & \textbf{3.91} \\

%     \bottomrule
%     \end{tabular}

%     \label{tab:ablation}
% \end{table*}

% \begin{table*}[!t]
%     \small
%     \centering
%     \caption{Ablation Study on Cube-Challenge. The best results are bold and the second best are underlined. }
%     \vspace{-1em}
%     \begin{tabular}{ccccc|c|c|ccccc}
%     \toprule
%     \multicolumn{5}{c|}{Contributions} & \# Param. & FLOPs  & Mean & Med. & Tri. & Best  & Worst  \\ \cline{0-4} 
%     Model & Backbone & Multi-Stages & ISAMs & Relighting &  &  & & & & 25\% & 25\% \\\hline
%     % FC4~\cite{hu2017fc4} & Random & \underline{1.70M} & \textbf{1.59G} & 1.97 & 1.24& 1.36 & 0.46 & 4.77\\
%     $\mathit{A}$ & FC4 & - & - & No Aug. & \underline{1.70M} & \textbf{1.59G} & 1.75 & 1.00 & 1.13 & 0.37 & 4.45\\
%     % FC4~\cite{hu2017fc4} & Proposed & \underline{1.70M} & \textbf{1.59G} & 1.61 & 0.95 & 1.01 & 0.33 & 4.14\\
%     % C4~\cite{yu2020c4}(Only pre-trained backbone) & w/o & 5.11M & 4.77G & N/A & N/A & N/A & N/A & N/A  \\
%     % C4~\cite{yu2020c4}(Finetune on FC4~\cite{hu2017fc4}) & Random & 5.11M & 4.77G & 1.84 & 1.11 & 1.25 & 0.38 & 4.54  \\ 
%     $\mathit{B}$ & FC4 & unshared & - & No Aug. & 5.11M & 4.77G & 1.84 & 1.11 & 1.26 & 0.44 & 4.53  \\ 
%     % C4~\cite{yu2020c4}(Finetune on FC4~\cite{hu2017fc4}) & Proposed & 5.11M & 4.77G & 1.62 & 1.01 & 1.07 & 0.38 & 4.03  \\ \hline
%     % $\mathit{C}$ & FC4 & shared & - & No Aug. & 1.70M & 4.77G & 1.75 & 1.00 & 1.10 & 0.33 & 4.54 \\
%     $\mathit{C}$ & FC4 & shared & - & No Aug. & 1.70M & 4.77G & 1.76 & 1.08 & 1.19 & 0.38 & 4.31 \\
%     % $\mathit{D}$ & FC4 & shared & shared & No Aug. & 1.75M & 4.77G & 1.84 & 1.09 & 1.20 & 0.35 & 4.67 \\
%     $\mathit{D}$ & FC4 & shared & shared & No Aug. & 1.75M & 4.77G & 1.72 & 1.09 & 1.14 & 0.33 & 4.31 \\
%     $\mathit{E}$ & FC4 & shared & unshared & No Aug. & 1.84M & 4.77G & 1.67 & 1.04 & 1.12 & 0.33 & 4.11 \\
%     $\mathit{F}$ & FC4 & shared & only last & No Aug. & 1.80M & 4.77G & 1.69 & 1.04 & 1.10 & 0.34 & 4.24 \\
%     $\mathit{G}$ & FC4 & shared & unshared & Random & 1.84M & 4.77G & 1.69 & 1.08 & 1.18 & \textbf{0.29} & 4.17 \\
%     % Share-C4 \& Unshare-ISAM~(Only Channel Attention) & w/o & 1.84M & 4.77G & 1.68 & 0.88 & 0.98 & 0.27 & 4.54 \\
%     $\mathit{H}$ & FC4 &  shared & unshared & Proposed & 1.84M & 4.77G & \underline{1.60} & \underline{0.93} & \textbf{1.01} & \textbf{0.29} & \underline{4.10} \\
%     $\mathit{I} $ & L-FC4 & shared & unshared & Proposed & \textbf{0.82M} & \underline{3.93G} & \textbf{1.57} & \textbf{0.91} & \underline{1.06} & \underline{0.31} & \textbf{3.91} \\

%     \bottomrule
%     \end{tabular}

%     \label{tab:ablation}
% \end{table*}



% \textbf{Effect on the Number of Training Samples.}
% Since data augmentation is widely-used when the training data are insufficient. One question is:~\textit{Does the proposed data augmentation technique work well on any amount of the training samples?} To answer this question, we train the FC4 network~\cite{hu2017fc4} with $k$~($k=100,400,700,1000,1300,1707$~(all images)) samples on the largest available \textit{single sensor} dataset~(Cube+~\cite{cube}) using different data augmentation methods. We evaluate the models on the Cube-Challenge dataset (363 test images regardless of different $k$), which is captured by the same sensor as the training dataset. 

% We compare the proposed relighting method with the previous random relighting~(Random) in \cite{hu2017fc4} and no-relighting~(No~Aug.) from several aspects. 
% As shown in Figures~\ref{fig:relighting_a}-\ref{fig:relighting_c}, our method demonstrates a significant advantage compared to random relighting and no-relighting on all the metrics~(Mean, Best 25\% and Worst 25\%) regardless of the number of training samples. We also find that for this training set Cube+ and test set Cube-Challenge, more training samples~($>$400) may not influence the performance a lot, but the proposed method still performs the best.

%especially when the size of the dataset is small~$(k=100)$, which shows the generalization ability of the proposed method when there are limited training data. The random label augmentation also helps to stabilize when the training samples are limited~(Figure~\ref{fig:relighting_c}). However, this method damages the performance when the dataset is larger. This is caused by the fact that the random label augmentation ignores the property of the camera.

% On the other hand, according to the worst 25\% of the angular errors in Figure~\ref{fig:relighting_c}, we argue that the proposed method can gain much more robust results compared with others because of the comprehensive usage of the training dataset, which is more useful in practical applications. We also show the training process in Figure~\ref{fig:relighting_d}. Although random relighting can also prevent overfitting and stabilize the training, it cannot boost the performance compared with no-relighting. Differently, our method can not only stabilize the training process but also get better performance.
% Besides, though the proposed method does not increase the Mean performance on the larger dataset~($k=700$,~Figure~\ref{fig:relighting_a}), it still obtains better Worst 25\% as shown in Figure~\ref{fig:relighting_c}.
% Interestingly, the proposed data augmentation increases the performance a little when given sufficient training samples~(K=700). So we argue the current Gehler-Shi dataset~(300+ for training) and NUS8~(100+ for training) are too small and larger dataset~(training sample larger than 700) are needed to be used for evaluation. 
% Another important phenomenon is that our method may obtain results similar to no-relighting on Best 25\% in some cases~(Figure~\ref{fig:relighting_b}). It might be because the von Kries assumption~\cite{von} is still too simple to cover all real-world scenarios.
%We also argue that better methods should be proposed to obtain more accurate ground-truth.
%Another reason might because the labels from the color checker are mixed with noise.

% * FC4 data augmentation can be used to squeeze the domain gap and add noise to training process.
% * Their methods may hurt the performance when there is only one sensor
% * The proposed methods can gain better results.


% \begin{table}[t]              
%     \centering
%     \caption{Ablation Study on MCC Dataset}
%     \begin{tabular}{l|c|ccccc}
%     \toprule
%     Method & Aug. & Mean & Med. & Tri. & Best & Worst \\
%      &  &  &  & Mean & 25\% & 25\%  \\
%     \hline
%     FC4\cite{hu2017fc4} & w/o & 1.76 & 1.15 & 1.27 & 0.34 & 4.23 \\
%     FC4\cite{hu2017fc4} & R & 1.65 & 1.18 & 1.27 & 0.38 & 3.78 \\
%     FC4\cite{hu2017fc4} & S+R & 1.53 & 1.07 & 1.13 & 0.30 & 3.63 \\ \hline
   
%     Ours & w/o & 1.69 & 1.21 & 1.28 & 0.37 & 3.87 \\
%     Ours &  R & 1.36 & 0.87 & 0.99 & 0.27 & 3.34 \\
%     Ours & S+R & 1.30 & 0.85 & 0.94 & \textbf{0.27} & 3.12 \\
  
%     \bottomrule
%     \end{tabular}

%     \label{tab:relighting}
% \end{table}
% \textbf{Intermediate} 







\begin{figure*}[t]
\centering
\begin{subfigure}{\xxwidth\textwidth}
    \centering
    \includegraphics[width=0.88\columnwidth]{figures/supp/iteations/canon550d1939_raw.jpg}
    \vspace{-0.4em}
    \caption*{Input}
\end{subfigure}
\begin{subfigure}{\xxwidth\textwidth}
    \centering
    \includegraphics[width=\columnwidth]{figures/supp/iteations/canon550d1939_s1.jpg}
    \vspace{-1.5em}
    \caption*{Stage1~($5.75^{\circ}$)}
\end{subfigure}
\begin{subfigure}{\xxwidth\textwidth}
    \centering
    \includegraphics[width=\columnwidth]{figures/supp/iteations/canon550d1939_s2.jpg}
    \vspace{-1.5em}
    \caption*{Stage2~($2.20^{\circ}$)}
\end{subfigure}
\begin{subfigure}{\xxwidth\textwidth}
    \centering
    \includegraphics[width=\columnwidth]{figures/supp/iteations/canon550d1939_s3.jpg}
    \vspace{-1.5em}
    \caption*{Stage3~($\mathbf{1.45^{\circ}}$)}
\end{subfigure}
\begin{subfigure}{\xxwidth\textwidth}
    \centering
    \includegraphics[width=\columnwidth]{figures/supp/iteations/canon550d1939_gt.jpg}
    \vspace{-1.5em}
    \caption*{Ground Truth}
\end{subfigure}

\begin{subfigure}{\xxwidth\textwidth}
    \centering
    \includegraphics[width=0.88\columnwidth]{figures/supp/iteations/canon550d2013_raw.jpg}
    \vspace{-0.4em}
    \caption*{Input}
\end{subfigure}
\begin{subfigure}{\xxwidth\textwidth}
    \centering
    \includegraphics[width=\columnwidth]{figures/supp/iteations/canon550d2013_s1.jpg}
    \vspace{-1.5em}
    \caption*{Stage1~($6.94^{\circ}$)}
\end{subfigure}
\begin{subfigure}{\xxwidth\textwidth}
    \centering
    \includegraphics[width=\columnwidth]{figures/supp/iteations/canon550d2013_s2.jpg}
    \vspace{-1.5em}
    \caption*{Stage2~($3.07^{\circ}$)}
\end{subfigure}
\begin{subfigure}{\xxwidth\textwidth}
    \centering
    \includegraphics[width=\columnwidth]{figures/supp/iteations/canon550d2013_s3.jpg}
    \vspace{-1.5em}
    \caption*{Stage3~($\mathbf{1.00^{\circ}}$)}
\end{subfigure}
\begin{subfigure}{\xxwidth\textwidth}
    \centering
    \includegraphics[width=\columnwidth]{figures/supp/iteations/canon550d2013_gt.jpg}
    \vspace{-1.5em}
    \caption*{Ground Truth}
\end{subfigure}


% \begin{subfigure}{\xxwidth\textwidth}
%     \centering
%     \includegraphics[width=0.88\columnwidth]{figures/supp/iteations/FujifilmXM1_0114_raw.jpg}
%     \vspace{-0.4em}
%     \caption*{Input}
% \end{subfigure}
% \begin{subfigure}{\xxwidth\textwidth}
%     \centering
%     \includegraphics[width=\columnwidth]{figures/supp/iteations/FujifilmXM1_0114_s1.jpg}
%     \vspace{-1.5em}
%     \caption*{Stage1~($6.11^{\circ}$)}
% \end{subfigure}
% \begin{subfigure}{\xxwidth\textwidth}
%     \centering
%     \includegraphics[width=\columnwidth]{figures/supp/iteations/FujifilmXM1_0114_s2.jpg}
%     \vspace{-1.5em}
%     \caption*{Stage2~($2.30^{\circ}$)}
% \end{subfigure}
% \begin{subfigure}{\xxwidth\textwidth}
%     \centering
%     \includegraphics[width=\columnwidth]{figures/supp/iteations/FujifilmXM1_0114_s3.jpg}
%     \vspace{-1.5em}
%     \caption*{Stage3~($\mathbf{1.02^{\circ}}$)}
% \end{subfigure}
% \begin{subfigure}{\xxwidth\textwidth}
%     \centering
%     \includegraphics[width=\columnwidth]{figures/supp/iteations/FujifilmXM1_0114_gt.jpg}
%     \vspace{-1.5em}
%     \caption*{Ground Truth}
% \end{subfigure}

% \begin{subfigure}{\xxwidth\textwidth}
%     \centering
%     \includegraphics[width=0.88\columnwidth]{figures/supp/iteations/SamsungNX2000_0132_raw.jpg}
%     \vspace{-0.4em}
%     \caption*{Input}
% \end{subfigure}
% \begin{subfigure}{\xxwidth\textwidth}
%     \centering
%     \includegraphics[width=\columnwidth]{figures/supp/iteations/SamsungNX2000_0132_s1.jpg}
%     \vspace{-1.5em}
%     \caption*{Stage1~($3.20^{\circ}$)}
% \end{subfigure}
% \begin{subfigure}{\xxwidth\textwidth}
%     \centering
%     \includegraphics[width=\columnwidth]{figures/supp/iteations/SamsungNX2000_0132_s2.jpg}
%     \vspace{-1.5em}
%     \caption*{Stage2~($2.18^{\circ}$)}
% \end{subfigure}
% \begin{subfigure}{\xxwidth\textwidth}
%     \centering
%     \includegraphics[width=\columnwidth]{figures/supp/iteations/SamsungNX2000_0132_s3.jpg}
%     \vspace{-1.5em}
%     \caption*{Stage3~($\mathbf{0.94^{\circ}}$)}
% \end{subfigure}
% \begin{subfigure}{\xxwidth\textwidth}
%     \centering
%     \includegraphics[width=\columnwidth]{figures/supp/iteations/SamsungNX2000_0132_gt.jpg}
%     \vspace{-1.5em}
%     \caption*{Ground Truth}
% \end{subfigure}


% \begin{subfigure}{\xxwidth\textwidth}
%     \centering
%     \includegraphics[width=0.88\columnwidth]{figures/supp/iteations/SonyA57_0249_raw.jpg}
%     \vspace{-0.4em}
%     \caption*{Input}
% \end{subfigure}
% \begin{subfigure}{\xxwidth\textwidth}
%     \centering
%     \includegraphics[width=\columnwidth]{figures/supp/iteations/SonyA57_0249_s1.jpg}
%     \vspace{-1.5em}
%     \caption*{Stage1~($2.23^{\circ}$)}
% \end{subfigure}
% \begin{subfigure}{\xxwidth\textwidth}
%     \centering
%     \includegraphics[width=\columnwidth]{figures/supp/iteations/SonyA57_0249_s2.jpg}
%     \vspace{-1.5em}
%     \caption*{Stage2~($1.13^{\circ}$)}
% \end{subfigure}
% \begin{subfigure}{\xxwidth\textwidth}
%     \centering
%     \includegraphics[width=\columnwidth]{figures/supp/iteations/SonyA57_0249_s3.jpg}
%     \vspace{-1.5em}
%     \caption*{Stage3~($\mathbf{0.79^{\circ}}$)}
% \end{subfigure}
% \begin{subfigure}{\xxwidth\textwidth}
%     \centering
%     \includegraphics[width=\columnwidth]{figures/supp/iteations/SonyA57_0249_gt.jpg}
%     \vspace{-1.5em}
%     \caption*{Ground Truth}
% \end{subfigure}



\begin{subfigure}{\xxwidth\textwidth}
    \centering
    \includegraphics[width=0.88\columnwidth]{figures/supp/iteations/NikonD5200_0195_raw.jpg}
    \vspace{-0.4em}
    \caption*{Input}
\end{subfigure}
\begin{subfigure}{\xxwidth\textwidth}
    \centering
    \includegraphics[width=\columnwidth]{figures/supp/iteations/NikonD5200_0195_s1.jpg}
    \vspace{-1.5em}
    \caption*{Stage1~($2.15^{\circ}$)}
\end{subfigure}
\begin{subfigure}{\xxwidth\textwidth}
    \centering
    \includegraphics[width=\columnwidth]{figures/supp/iteations/NikonD5200_0195_s2.jpg}
    \vspace{-1.5em}
    \caption*{Stage2~($1.17^{\circ}$)}
\end{subfigure}
\begin{subfigure}{\xxwidth\textwidth}
    \centering
    \includegraphics[width=\columnwidth]{figures/supp/iteations/NikonD5200_0195_s3.jpg}
    \vspace{-1.5em}
    \caption*{Stage3~($\mathbf{0.62^{\circ}}$)}
\end{subfigure}
\begin{subfigure}{\xxwidth\textwidth}
    \centering
    \includegraphics[width=\columnwidth]{figures/supp/iteations/NikonD5200_0195_gt.jpg}
    \vspace{-1.5em}
    \caption*{Ground Truth}
\end{subfigure}

\begin{subfigure}{\xxwidth\textwidth}
    \centering
    \includegraphics[width=0.88\columnwidth]{figures/supp/iteations/PanasonicGX1_0183_raw.jpg}
    \vspace{-0.4em}
    \caption*{Input}
\end{subfigure}
\begin{subfigure}{\xxwidth\textwidth}
    \centering
    \includegraphics[width=\columnwidth]{figures/supp/iteations/PanasonicGX1_0183_s1.jpg}
    \vspace{-1.5em}
    \caption*{Stage1~($1.77^{\circ}$)}
\end{subfigure}
\begin{subfigure}{\xxwidth\textwidth}
    \centering
    \includegraphics[width=\columnwidth]{figures/supp/iteations/PanasonicGX1_0183_s2.jpg}
    \vspace{-1.5em}
    \caption*{Stage2~($0.61^{\circ}$)}
\end{subfigure}
\begin{subfigure}{\xxwidth\textwidth}
    \centering
    \includegraphics[width=\columnwidth]{figures/supp/iteations/PanasonicGX1_0183_s3.jpg}
    \vspace{-1.5em}
    \caption*{Stage3~($\mathbf{0.12^{\circ}}$)}
\end{subfigure}
\begin{subfigure}{\xxwidth\textwidth}
    \centering
    \includegraphics[width=\columnwidth]{figures/supp/iteations/PanasonicGX1_0183_gt.jpg}
    \vspace{-1.5em}
    \caption*{Ground Truth}
\end{subfigure}

\caption{The intermediate results in different stages of the proposed network. The images are taken from Cube-Challenge and NUS8. Note that the calibration objects are masked out when training and testing.}
\vspace{1em}
\label{fig:iteration}
\end{figure*}




\begin{table*}[!t]
    \small
    \centering
    \caption{Ablation Study of the network structure on Cube-Challenge. The best results are bold and the second best are underlined. }
   
    \begin{tabular}{ccccc|c|c|ccccc}
    \toprule
    \multicolumn{5}{c|}{Contributions} & \# Param. & FLOPs  & Mean & Med. & Tri. & Best  & Worst  \\ \cline{0-4} 
    Model & Backbone & Multi-Stages & ISAMs & Aug. &  &  & & & & 25\% & 25\% \\\hline
    % FC4~\cite{hu2017fc4} & Random & \underline{1.70M} & \textbf{1.59G} & 1.97 & 1.24& 1.36 & 0.46 & 4.77\\
    % $\mathit{A}$ & FC4 & - & - & No Aug. & \underline{1.70M} & \textbf{1.59G} & 1.75 & 1.00 & 1.13 & 0.37 & 4.45\\
    % FC4~\cite{hu2017fc4} & Proposed & \underline{1.70M} & \textbf{1.59G} & 1.61 & 0.95 & 1.01 & 0.33 & 4.14\\
    % C4~\cite{yu2020c4}(Only pre-trained backbone) & w/o & 5.11M & 4.77G & N/A & N/A & N/A & N/A & N/A  \\
    % C4~\cite{yu2020c4}(Finetune on FC4~\cite{hu2017fc4}) & Random & 5.11M & 4.77G & 1.84 & 1.11 & 1.25 & 0.38 & 4.54  \\ 
    $\mathit{A}$ & FC4 & unshared & - & - & 5.11M & 4.77G & 1.84 & 1.11 & 1.26 & 0.44 & 4.53  \\ 
    % C4~\cite{yu2020c4}(Finetune on FC4~\cite{hu2017fc4}) & Proposed & 5.11M & 4.77G & 1.62 & 1.01 & 1.07 & 0.38 & 4.03  \\ \hline
    % $\mathit{C}$ & FC4 & shared & - & No Aug. & 1.70M & 4.77G & 1.75 & 1.00 & 1.10 & 0.33 & 4.54 \\
    $\mathit{B}$ & FC4 & shared & - & - & 1.70M & 4.77G & 1.76 & 1.08 & 1.19 & 0.38 & 4.31 \\
    % $\mathit{D}$ & FC4 & shared & shared & No Aug. & 1.75M & 4.77G & 1.84 & 1.09 & 1.20 & 0.35 & 4.67 \\
    $\mathit{C}$ & FC4 & shared & shared & - & 1.75M & 4.77G & 1.72 & 1.09 & 1.14 & 0.33 & 4.31 \\
    $\mathit{D}$ & FC4 & shared & unshared & - & 1.84M & 4.77G & 1.66 & 0.95 & \textbf{1.03} & \textbf{0.29} & 4.29 \\
    $\mathit{E}$ & FC4 & shared & only last & - & 1.80M & 4.77G & 1.69 & 1.04 & 1.10 & 0.34 & 4.24 \\
    % $\mathit{G}$ & FC4 & shared & unshared & Random & 1.84M & 4.77G & 1.69 & 1.08 & 1.18 & \textbf{0.29} & 4.17 \\
    % Share-C4 \& Unshare-ISAM~(Only Channel Attention) & w/o & 1.84M & 4.77G & 1.68 & 0.88 & 0.98 & 0.27 & 4.54 \\
    $\mathit{F}$ & L-FC4 & shared & unshared & - & \underline{0.82M} & \underline{3.93G} & 1.64 & \underline{0.92} & \underline{1.04} & 0.33 & 4.25 \\
    \hline
    $\mathit{G}$~(final) & L-FC4 & shared & unshared & SIE & \underline{0.82M} & \underline{3.93G} & \textbf{1.57} & \textbf{0.91} & 1.06 & \underline{0.31} & \textbf{3.92} \\ \hline
    
    $\mathit{H}$ & L-FC4-G & shared & unshared & SIE & \textbf{0.66M} & \textbf{3.87G} & 1.63 & 1.04 & 1.12 & 0.32 & \underline{3.97} \\
    $\mathit{I} $ & L-FC4-L & shared & unshared & SIE & \textbf{0.66M} & \underline{3.93G} & \underline{1.62} & 0.96 & 1.06 & 0.32 & 4.10 \\
    
    \bottomrule
    \end{tabular}
    \label{tab:ablation}
\end{table*}



\begin{figure}[t]
\centering
\includegraphics[width=1\linewidth]{IEEEtran/figures/all.pdf}
\caption{Effect of shared/unshared attentions. (a) and~(b) show the activation distributions of the first channel re-calibration in the shared and unshared ISAMs in Model~$\mathit{C}$ and Model~$\mathit{D}$ from a single image, respectively. The unshared attentions activate more channels to learn the illuminant differences in each stage, while most activations of different stages are similar in the shared attentions. In (a), ALL of the activations from stages 2 and 3 are overlapped.}
\label{fig:att}
\end{figure}


% \begin{figure}[t]
% \centering
% \begin{subfigure}[t]{0.9\columnwidth}
%   \includegraphics[width=1\linewidth]{IEEEtran/figures/all.pdf}
%   \caption{Shared Attentions}
%   \label{fig:Ng1} 
% \end{subfigure}
% \\
% \begin{subfigure}[t]{0.9\columnwidth}
%   \includegraphics[width=1\linewidth]{IEEEtran/figures/unshare.pdf}
%   \caption{Unshared Attentions}
%   \label{fig:Ng2}
% \end{subfigure}
% \caption{Effect of shared/unshared attentions. (a) and~(b) show the activation distributions of the first channel re-calibration in the shared and unshared ISAMs in Model~$\mathit{C}$ and Model~$\mathit{D}$ from a single image, respectively. The unshared attentions activate more channels to learn the illuminant differences in each stage, while most activations of different stages are similar in the shared attentions. In (a), ALL of the activations from stages 2 and 3 are overlapped.}
% \label{fig:att}
% \end{figure}


% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\columnwidth]{figures/canon550d1740.png}

%     \caption{Effect of shared/unshared attentions. (a) and~(b) show the activation distributions of the first channel re-calibration in the shared and unshared ISAMs in Model~$\mathit{C}$ and Model~$\mathit{D}$ from a single image, respectively. The unshared attentions activate more channels to learn the illuminant differences in each stage, while most activations of different stages are similar in the shared attentions. In (a), most of the activations from stages 2 and 3 are overlapped.}

%     \label{fig:att}
% \end{figure}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\columnwidth]{figures/canon550d1740.png}

%     \caption{Effect of shared/unshared attentions. (a) and~(b) show the activation distributions of the first channel re-calibration in the shared and unshared ISAMs in Model~$\mathit{C}$ and Model~$\mathit{D}$ from a single image, respectively. The unshared attentions activate more channels to learn the illuminant differences in each stage, while most activations of different stages are similar in the shared attentions. In (a), most of the activations from stages 2 and 3 are overlapped.}

%     \label{fig:att}
% \end{figure}


% \begin{figure}[t]
% \centering
% \includegraphics[width=1\columnwidth]{IEEEtran/figures/all.pdf}
% \caption{Effect of shared/unshared attentions. (a) and~(b) show the activation distributions of the first channel re-calibration in the shared and unshared ISAMs in Model~$\mathit{C}$ and Model~$\mathit{D}$ from a single image, respectively. The unshared attentions activate more channels to learn the illuminant differences in each stage, while most activations of different stages are similar in the shared attentions. In (a), ALL of the activations from stages 2 and 3 are overlapped.}
% \label{fig:att}
% \end{figure}

\subsection{Ablation Study of the Network Structure} 
\label{sec:exp_net}
We have proposed a compact cascaded framework which shares the backbone in three cascaded stages and learns each stage specifically by the proposed \textit{Iteration-Specific Attention Module}~(ISAM). In this section, we do the ablation study of each component in the proposed framework on Cube-Challenge~\cite{cubechallenge}, since the NUS8 and Gehler-Shi datasets are relatively small.  
As shown in Table~\ref{tab:ablation}, we start with the baseline~(Model~$\mathit{A}$, C4~\cite{yu2020c4}, \ie,~using three unshared FC4~\cite{hu2017fc4} backbones) without the sensor-aware illuminant enhancement~(SIE). Because of the heavy network structure, directly training the cascaded network without SIE shows an unsatisfactory result compared to the model that shares the backbone in all stages~(Model~$\mathit{B}$). If we add ISAMs to Model~$\mathit{B}$ and share them in different stages~(Model~$\mathit{C}$), the network only performs slightly better on some metrics than Model~$\mathit{B}$ due to extra parameters added. Differently, when we learn the ISAMs specifically~(Model~$\mathit{D}$), all the metrics are improved significantly, which confirms the observation that the distributions in multiple stages are different and should be learnt specifically. We compare the activations of channel re-calibration in each stage between Model~$\mathit{C}$ and Model~$\mathit{D}$ in Figure~\ref{fig:att}. 
The unshared attentions show a much denser activation map in different stages while the shared attentions are insensitive to the changes of the illuminant especially in stages 2 and 3.

Besides, we also test the model when there is only the last ISAM in each stage~(Model~$\mathit{E}$). The performance of Model~$\mathit{E}$ drops a little but is still better than Model~$\mathit{B}$ and Model~$\mathit{C}$ that have either no attention or shared attentions. Then, if we replace the backbone FC4 with our dual-branch lightweight L-FC4~(Model~$\mathit{F}$), we get better overall performance than Model~$\mathit{D}$ but use only half of the parameters. And in Model~$\mathit{G}$, the usage of SIE also increases the performance of the network a lot. % of our network



Next, we evaluate each branch of the proposed dual-branch lightweight head in Models~$\mathit{H}$~and~$\mathit{I}$~(as shown in Figure~\ref{fig:head}). Although the local branch~(L-FC4-L) and the global branch~(L-FC4-G) based models can further reduce the parameters, their performances are worse than Model~$\mathit{G}$ that has both branches. 

Finally, in Figure~\ref{fig:iteration}, we give the intermediate illuminants, corrected images and angular errors from the multiple stages~(iterations) of the proposed network to prove the effectiveness of the cascaded framework. We discover that using more stages gains much better performance than using only one stage. However, four or more stages may not improve~\cite{yu2020c4}, so in all our experiments we choose the number of stage equal to 3.
%The proposed network builds on C4~\cite{yu2020c4} and FC4~\cite{hu2017fc4}, but performs more accurately and efficiently thanks to lightweight head and iteration-aware attention modules. 
% As shown in Table~\ref{tab:ablation}, we first evaluate the performance of the proposed assumption of iteration-aware attention~(ISAM) with the same network but shared attention~(Share-AM), where the proposed framework attention performs much better performance but only needs few parameters. We also give the attention maps in Figure~\ref{fig:att_vis} to show the effect of iteration-aware attentions among stages, where the attended pixels and channels are different.
% Then, we replace the multi-scale ISAM from the proposed method in each Max-Pooling layer with the last one in each stage, the degraded performance confirms the contribution. 
% We also evaluate the performances of each relighting augmentation methods on the proposed network in table, where the proposed relighting method also works well in this dataset and the proposed methods.
% Finally, we do the ablation study on the proposed lightweight head. From the table, compared with the original FC4~\cite{hu2017fc4}, the proposed lightweight head reduces half of the parameters but gains better results. 
% And also, compared with C4~\cite{yu2020c4}, the fully proposed method reduce nearly 80\% of the parameters and 20\% of the FLOPs.

% Notice that, by parameters sharing, all the proposed structures (Model~$\mathrm{C-I}$) can be trained with only initializing from the pretrained ImageNet backbone, while C4~\cite{yu2020c4} requires to initialize the stages using the same parameters from the pre-trained one stage~(Model~$\mathrm{A}$) and fine-tune on their cascaded framework. We have tested several datasets~(including Gehler-Shi and Cube-Challenge, NUS8~(\textit{Sony}, \textit{Samsung})), C4~\cite{yu2020c4} always fails without the single stage pre-training. 


% \begin{table}[!t]
%     \small
%     \centering
%     \caption{Ablation Study on Network Structure}
%     \vspace{-1em}
%     \begin{tabular}{l|c|c|ccccc}
%     \toprule
%     Model & \# Pa. & MFLPs  & Mean & Med. & Tri. & Bst  & Wst  \\
%     &  &  &  &  & & 25\% & 25\% \\\hline
%     FC4~\cite{hu2017fc4} & 1.7M & 1.59G & 1.65 & 1.18 & 1.27 & 0.38 & 3.78 \\
%     C4(scratch)\cite{yu2020c4} &  4.8M & 4.77G & n/a & n/a & n/a & n/a & n/a  \\
%     C4(finetune)\cite{yu2020c4} & 4.8M & 4.77G & 1.35 & 0.88 & 0.99 & 0.28 & 3.21 \\
%     C4(Model F)\cite{yu2020c4} & 1.7M & - & 1.47 & 0.97 & 1.09 & 0.31 & 3.49 \\\hline

%     S-C4+att  & 1.7M & & 1.41 & 0.98 & 1.08 & 0.30 & 3.28 \\
%     S-C4+att   & 1.8M & & 1.34 & 0.84 & 0.95 & 0.29 & 3.23 \\
%     S-C4+att+LIP & 0.7M & & 1.37 & 0.92 & 1.01 & 0.28 & 3.30 \\
%     S-C4+att+MSH & 0.8M & & 1.30 & 0.85 & 0.94 & \textbf{0.27} & 3.12 \\
%     S-C4+MSH  & 0.6M &  & 1.57 & 1.11 & 1.19 & 0.33 & 3.63 \\
%     Full method & 0.8M & 3.93G & \textbf{1.27} & \textbf{0.81} & \textbf{0.90} & 0.28 & \textbf{3.04} \\
    
%     % Shared C4 + MSH & 0.7M & S+R & 1.57 & 1.11 & 1.19 & 0.33 & 3.63 \\
    
%     \bottomrule
%     \end{tabular}

%     \label{tab:ablation}
% \end{table}


% \subsubsection{Loss Function}
% \subsubsection{Ablation Study on Loop performance}
% \subsubsection{Ablation Study on Inference Time}
% Since our network use much few parameters by recurrently attention module, the main drawback is the inference time. Here, we compare the inference time with the previous state-of-the-art methods. 

% \begin{itemize}
%     \item our 0.05s 0.04754328727722168
%     \item ECA 0.01493072509765625
%     \item C1 0.003s
%     \item C4 0.014s
%     \item ECA(stage=2) 0.010797739028930664
% \end{itemize}



% \begin{figure}
% \centering
% \begin{subfigure}[b]{0.45\textwidth}
%   \includegraphics[width=1\linewidth]{figures/share_attention.jpg}
%   \vspace{-2em}
%   \caption{Shared Attentions}
%   \label{fig:atta} 
% \end{subfigure}

% \begin{subfigure}[b]{0.45\textwidth}
%   \includegraphics[width=1\linewidth]{figures/our_attention.jpg}
%     \vspace{-2em}
%   \caption{Unshared Attentions}
%   \label{fig:attb}
% \end{subfigure}
% \vspace{-1em}
% \caption{Effect of unshared/shared attentions. (a) and (b) show the activations in the first channel recalibration in shared ISAM~(Model~$\mathit{D}$) and unshared ISAM~(Model~$\mathit{E}$), respectively. Unshared attentions activate more channels to learn the differences in each stage, while most activations of different stages are similar in shared attentions. In (a), nearly all the activations from stages 2 and 3 are overlapped.}\label{fig:att}
% \end{figure}

% \begin{figure}[t!]
%     \centering
%     \begin{subfigure}[t]{\columnwidth}
%         \begin{minipage}[b]{\textwidth}
%         \includegraphics[width=\textwidth]{figures/share_attention.jpg}
%         \end{minipage}
%         \vspace{-2em}
%         \caption{Shared Attentions}
%         \label{fig:atta}
%     \end{subfigure}%
%     \begin{subfigure}[t]{\columnwidth}
%     \begin{minipage}[b]{\textwidth}
%         \includegraphics[width=\textwidth]{figures/our_attention.jpg}
%         \end{minipage}
%         \vspace{-2em}
%         \caption{Unshared Attentions}
%         \label{fig:attb}
%     \end{subfigure}
%     \vspace{-0.8em}
%     \caption{Effect of unshared/shared attentions. (a) and (b) show the activations in the first channel recalibration in shared ISAM~(Model~$\mathit{D}$) and unshared ISAM~(Model~$\mathit{E}$), respectively. Unshared attentions activate more channels to learn the differences in each stage, while most activations of different stages are similar in shared attentions. In (a), nearly all the activations from stages 2 and 3 are overlapped.}
%     \label{fig:att}
% \end{figure}

% todo: add more discussions on the label shuffle




==> IEEEtran/subfiles/introduction.tex <==
%%%%%%%%% ABSTRACT


\section{Introduction}

% Automatically color consistency is a fundamental problem in  computer vision community. In traditional methods, edges and gray pixels plays a critical role in this task.
% Recently, deep learning based methods also draw the attention from the community since several years ago~\cite{ccc,ffcc,dsn}.

% The color captured by cameras is often baised because of the ext  

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\columnwidth]{figures/teast.png}
%     \vspace{-2em}
%     \caption{A glance of the proposed training method. Because of the existence of camera spectral sensitivity, the illuminants captured by  different sensors are often different in the  $[\frac{G}{B}, \frac{G}{R}]$ color space. According to this property, the proposed method obtains the white-balanced image by the annotated \textit{ground-truth} illuminant~(label) and then relight it by the \textit{novel illuminants} from \textit{the same sensor} as the new training samples. Thus, we enlarge the dataset without any additional information, resulting in better results. The upper-left figure exhibits the illuminant distribution of images captured by \textit{Canon 5D} in Gehler-Shi dataset~\cite{shi2000re}. The images are applied with gamma correction for better visualization.}
%     \label{fig:reshuffle}
% \end{figure}

% what is the color constancy
\IEEEPARstart{H}{uman} vision system has a strong ability to perceive relatively constant colors of objects under varying illumination. However, it is difficult for digital cameras to have the same ability. In computer vision, this problem is formulated as computational Color Constancy~(CC), which is also a practical concern for the automatic white balance~(AWB)~\cite{ffcc}.
%In AWB, the camera needs to reproduce the original scene colors regarding the property of camera. 
Besides visual aesthetics, accurate white balance is also necessary for high-level tasks~\cite{Afifi_2019_ICCV}, such as image classification and semantic segmentation.
%also known as Automatic White Balance~(AWB) or scene illumination estimation, is a fundamental problem in computational photography. 
% The observation and methods of the proposed paper
%Different from previous works which often focus on designing a network structure or feature, in this paper, we give the discussion from a rare but important direction in this task by \textit{relighting}. 
% traditional method and their problem

\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\columnwidth]{IEEEtran/figures/mainpage.pdf}
    \caption{Our method utilizes the white-balanced images for cross sensor CC. Specifically, we consider unprocessed sRGB images~($I_{uip}$) and the corrected RAW images~($I_{awb}$) from real sensors as sensor-free white-balanced images. Then, we utilize these images and randomly sampled illuminants $\ell_{r}$ to train the network according to Eq.~\ref{eq:cc}.}

    \label{fig:xcc}
\end{figure}

In general, a photographed scene image $I_{raw}$ of color channel $c$, $I_{raw}^c$, can be represented as:
\begin{equation}
    I_{raw}^c(x) = \int_{\omega} E(\lambda,x)S(\lambda,x)C_c(\lambda)d\lambda,\quad  c \in \{r, g, b\},
    \label{eq:original}
\end{equation}
where $\omega$ is the visible light spectrum, and $x$ is the spatial location. At wavelength $\lambda$, $C_c(\lambda)$ is the camera sensor sensitivity~(CSS) function, $E(\lambda,x)$ and $S(\lambda,x)$ are the color of light source and the surface spectral reflectance, respectively. Assuming there is only one uniform illuminant in the scene, according to the von Keris model~\cite{von}, the above formula can be simplified as:
\begin{equation}
    I_{raw}^{c} =  I_{awb}^{c} \times \ell^{c} ,\quad c \in \{r, g, b\},
    \label{eq:cc}
\end{equation}
where $I_{awb}^{c}$, and $\ell^{c}$ are the channel $c$ of the corrected white balanced image and the scene illuminant, respectively. In practice, to acquire ground truth illumination for correction or training, a standard object with known chromatic properties~(\eg, color checker~\cite{shi2000re} or SpyderCube~\cite{cube}) often needs to be  placed into the scene. Thus, labelling a large-scale dataset for training a deep neural network is costly. Besides, since there are only 0.2k--0.3k images per sensor in the popular benchmarks~\cite{nus8,shi2000re}, the changes of surface spectral reflectance and color temperature are also insufficient for deep learning. 
Also because of the domain gap between sensors, most previous methods~\cite{hu2017fc4,bianco2015color,ffcc} can only work well for a specific sensor with the models trained on the same sensor.
% Since it has a long history in computer vision and color science, there have been many works to tackle this problem including statistics-based methods~\cite{gray-edge,gray-index,gray-world} and learning-based methods~\cite{ffcc,hu2017fc4,ccc,yu2020c4}. 
% However, modern deep learning-based color constancy algorithms also rely on the color $uv$-histogram~\cite{siie,ffcc,ccc} or heavy network structures~\cite{yu2020c4,hu2017fc4,end2end}. 
% According to this property, FC4~\cite{hu2017fc4} relights the raw image and its corresponding label by a random factor for data augmentation. However, the random label augmentation breaks the distribution of the illuminates as discussed. Also inspired by Eq.~\ref{eq:cc}, C4~\cite{yu2020c4} corrects the image via the prediction of FC4~\cite{hu2017fc4} and cascades it multiple times for coarse-to-fine prediction. Although C4 obtains state-of-the-art accuracy, the parameters in this model also increase multiple times when cascading multiple networks. 

To overcome aforementioned problems, as shown in Figure~\ref{fig:xcc}, we first propose a novel training technique, called \textit{self-supervised cross-sensor training}, to utilize the knowledge from the images from out-of-domain sensors, and even processed sRGB images. In detail, on the one hand,  we firstly consider the available sRGB datasets as white-balanced because these datasets are carefully corrected by humans or digital cameras. Then, we unprocess the sRGB images and sample the sensor-independent illuminants for training. On the other hand, we collect labelled images from several  sensors and correct the images via Eq.~\ref{eq:cc}. And then, for each white-balanced image, a new illuminant is randomly sampled to relight the image as supervision. Besides the training technique, we design a compact cascaded network based on C4~\cite{yu2020c4}. Considering each iteration in C4 as a residual distribution, we share the parameters in each iteration but learn the illuminant differences with a proposed \textit{iteration-specific attention module}.
Besides, different from C4 which uses FC4~\cite{hu2017fc4} as the backbone, we design a novel \textit{lightweight head} to replace the head in FC4~\cite{hu2017fc4}, reducing 50\% of the parameters while keeping accuracy. 

Our main contributions are summarized as follows:

\begin{itemize}
\item We propose \textit{self-supervised cross-sensor training} to obtain scene knowledge from abundant sRGB images and other available labelled RAW datasets. Once trained using randomly generated labels, our model achieves state-of-the-art performance on cross-sensor evaluation.

\item We design a novel and compact cascaded network structure via an \textit{iteration-specific attention module} and a \textit{lightweight multi-scale head}. 

% \item We involve the adaptive parameters learning as loss function to get more accurate results among the iteration.

\item Our single-sensor model achieves state-of-the-art performance on multiple popular datasets using only 16\% of the parameters of the existing best model~\cite{yu2020c4}.

\end{itemize}





==> IEEEtran/subfiles/method.tex <==
\section{Method}

Traditionally, CC has widely been explained as a supervised learning problem~\cite{hu2017fc4,yu2020c4}. 
Given a neural network $\psi(I_{raw}; \omega)$ with a raw image $I_{raw}$ as input, the network only predicts a globally three-dimensional normalized vector $\ell_{pred}$ representing the chromatism caused by corresponding illumination. Then, under the supervision of the ground-truth label~$\ell$ from manual acquisition, the parameters of the network $\omega$ are optimized by gradient descent. To simplify the notation in our analysis, we represent the basic training pair~(input,~label) for the white-balanced image $I_{awb}$ as:
\begin{equation}
    I_{awb} \Leftarrow (I_{raw},\ell).
    \label{eq:awb}
\end{equation}
% To simplify the notation in our analysis, we represent the basic training pair~(input,~label) for the white-balanced image $I_{awb}$ as:
% \begin{equation}
%     I_{awb} \Leftarrow (I_{raw},\ell).
%     \label{eq:awb}
% \end{equation}
% Based on Eq.~\ref{eq:cc} and Eq.~\ref{eq:awb}, we analysis the proposed methods starting from a nearly new viewpoint for learning-based CC via sensor-aware relighting. 
In this work, we find that the diversity of illuminants in datasets is the key to train a cross-sensor CC model and to improve the model performance for single-sensor CC. We propose a method to learn enriched illuminants for cross and single sensor CC. 
Firstly, we propose a self-supervised training technique to train a model for cross-sensor CC~(Sec.~\ref{sec:ss}). Secondly, the trained cross-sensor model can be further fine-tuned on the novel single sensor using the sensor-aware illuminant enhancement~(Sec.~\ref{sec32}).
Thirdly, as for the model design, we utilize the cascaded structure as a relighting-based label augmentation method which is different from C4~\cite{yu2020c4}, and propose a more compact and accurate model~(Sec.~\ref{sec:ccn}). 
Finally, the loss function we used is discussed in Sec.~\ref{sec:loss}.
Below, we give the detail of each part.




\subsection{Self-Supervised Cross-Sensor Training}
\label{sec:ss}
% It is ill-posed to gain the ground truth illumination from a single image without any hint. Thus, to get the real color from the scenes, color constancy dataset needs to place a Color Checker~\cite{wiki:cc} or other similar reference into the scene and correct it manually. Also,

%Finally, for AWB, the white-balanced image $I_{awb}$ can be obtained by Eq.~\ref{eq:cc}.

From Eq.~\ref{eq:original}, the white-balanced image is highly related to the CSS~\cite{siie,css,csswacv}, which describes the spectral response caused by a sensor and is typically different between sensors. Also, because of the existence of CSS, collecting a common large-scale labelled dataset for universal~(cross-sensor) CC is unrealistic. Besides, since the datasets are often collected in certain environments, the diversity of the illuminants is also limited~\cite{multi-hyp,oh2017approaching}. 
Thus, leveraging large-scale \textit{sensor-free} knowledge to 
train a deep network is important and necessary in CC. 

Inspired by recent development of self-supervised learning in image colorization~\cite{zhang2016colorful}, in-painting~\cite{deepfill} and machine translation~\cite{bert}, we propose a novel self-supervised cross-sensor training technique including two steps to tackle above issues. 
In detail, we utilize the white-balanced samples generated by unprocessing sRGB images to the RAW domain or correcting RAW images with corresponding labels from multiple sensors. And then we train a cross-sensor model with these images and randomly sampled illuminants. Below, we give the details of each step.
%Self-supervised learning, which generates the supervision from the images itself, has been recently succeed applied . As for color constancy, , 

\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\columnwidth]{IEEEtran/figures/uip.pdf}

    \caption{The relation among $I_{raw}$, $I_{awb}$, $I_{uip}$ and $I_{srgb}$ images. After AWB, $I_{raw}$ becomes $I_{awb}$. $I_{uip}$ is obtained by unprocessing an sRGB image~$I_{srgb}$, and is also white-balanced.}

    \label{fig:homo}
\end{figure}

\textbf{Unprocessing sRGB Images for Pre-Training~(UIP).} Since there are millions of well-processed sRGB images available ~\cite{deng2009imagenet,coco}, we treat these sRGB images as white-balanced and unprocess \cite{unprocessing} them to the RAW domain. Differently, since we consider the processed sRGB images are sensor-independent and white-balanced, we only do the inverse tone mapping and de-gamma correction to avoid the color change. Figure~\ref{fig:homo} shows the relation between an sRGB image $I_{srgb}$ and its unprocessed version $I_{uip}$. Then, we regard these images $I_{uip}$ as sensor-free white-balanced samples and randomly sample illuminants within a large range for generating training data. For example, since most of RAW images are in Bayer pattern~($RGGB$), we randomly sample an illuminant $\ell^c_{r} \in [0.2,0.8], c \in \{r,g,b\}$, double the green component and normalize the illuminant as ground truth for each image. Then, a new training combination $I_{uip} \Leftarrow (I_{raw},\ell_{r})$ can be obtained by $I^c_{raw} = I_{uip}^c \times \ell^c_{r}, c \in \{r,g,b\}$, according to Eq.~\ref{eq:cc}. Even if
these generated images may not represent real illuminants in the real world, the proposed method provides an almost unbiased dataset with countless synthesized illuminants for training and involves millions of available sRGB images.

After obtaining a large set of training pairs~(combinations), we train our network with it for the initialization of the network, which will be fine-tuned in the next step SAF.


\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{IEEEtran/figures/structure.pdf}

    \caption{The proposed network structure. The SqueezeNet backbone and the proposed \textit{Lightweight Head} for prediction are shared, and the \textit{Iteration-Specific Attention Module} is learnt specifically in each iteration. The ReLU layer is omitted after each convolutional layer for clarity.}

    \label{fig:nn}
\end{figure*}



\textbf{Sensor Alignment Fine-Tuning~(SAF).} Besides UIP, to match the distribution of real sensors for cross-sensor evaluation, we perform a similar self-supervised method on a dataset including multiple real sensors~\cite{laakom2019intel}. For fine-tuning, we firstly load the network parameters from the previous step UIP for the initialization. Then,
we correct the raw images $I_{raw}$ from each sensor by their corresponding ground-truth illumination labels $\ell$ using Eq.~\ref{eq:cc} to generate the sensor-free white-balanced images $I_{awb}$. Finally, we fine-tune the network with the samples and randomly sampled illuminants. Experiments show that our fine-tuned model can work well for \textit{novel sensor evaluation without fine-tuning on specific sensor data}. 



\subsection{Sensor-Aware Illuminant Enhancement for Single-Sensor Training}
% \label{sec:ss}
\label{sec32}
% In detail, following , Hu~\etal~\cite{hu2017fc4} use three independent factors~($ \xi = \xi_r, \xi_g, \xi_b$) for relighting on the raw image $I_{raw}$ and the ground-truth illumination $\ell$. Then, these augmented samples are used to train the neural network~\cite{hu2017fc4,mdlcc,yu2020c4}. This method is formulated as $I_{raw} \times \xi =  I_{awb} \times \ell \times \xi$. The new training process becomes $I_{awb} \Leftarrow ( I_{raw} \times \xi, \ell \times \xi ) $, where $ I_{raw} \times \xi$ and $ \ell \times \xi$ are the relighted images and illuminations, respectively. With different random independent factors $\xi$, compared to the training with Eq~\ref{eq:awb}, this method enlarges the dataset greatly.
% However, random relighting ignores the color distribution caused by CSS. As shown in Figure~\ref{fig:cdb}, we plot the randomly relighted samples in one epoch and impossible illuminations are introduced to the original sensors. Even the randomly augmented training samples will cover the whole space as the training epoch goes on. In this case, the network will try to fit the incorrect distribution. However, without the relighting for data augmentation, 

% Based on the previous cross domain model obtained by UP and SAF, we further fine-tune it for single-sensor CC, 
For single-sensor CC training, we also improve the performance by synthesizing illuminants that follow the distribution of the sensor's CSS similar to \cite{fourure2016mixed,lou2015color,hu2017fc4}. In detail, we first correct the RAW images $I_{raw}$ by their corresponding ground-truth illumination labels $\ell$ according to Eq.~\ref{eq:cc}. Then, new training samples are generated by randomly selected illuminants $\ell^\dag$ from the available data of the \textit{corresponding sensor}, which can be formulated as: $ \frac{I_{raw}}{\ell} \times \ell^\dag =  I_{awb} \times \ell^\dag,$ where we can train the network using the new combinations $I_{awb} \Leftarrow ( \frac{I_{raw}}{\ell} \times \ell^\dag, \ell^\dag)$. We name this scene relighting method as \textit{sensor-aware label reshuffle}~(Reshuffle).

Although Reshuffle can be used solely during training to improve performance for a specific sensor, we further combine random relighting\footnote{Similar to~\cite{hu2017fc4}, we rescale the images and corresponding labels by random RGB values in [0.6, 1.4], and normalize the results.} and the original training pairs to train the network alternatively on the fly for single-sensor CC, because it has been shown that training the network with some noise can also increase performance and stabilize the training process~\cite{sukhbaatar2014training,zhou2019towards}. We call 
our hybrid solution \textit{sensor-aware illuminant enhancement}~(SIE) and give the detailed analysis in the experiments. 


\subsection{Compact Cascaded Network}
\label{sec:ccn}
As for the network, we start with the previous work FC4~\cite{hu2017fc4} and C4~\cite{yu2020c4} due to their roles as the backbone and baseline for our work, respectively. In detail, FC4 uses the first 12 layers of the pre-trained SqueezeNet~\cite{squeezenet} as the feature extractor and two convolutional layers with confidence-weighted pooling to estimate the illuminant. Then, C4 cascades FC4 multiple times by correcting the input via Eq.~\ref{eq:cc}. Denoting a single stage C4 with parameters $\omega$ as $\psi(;\omega)$, we formulate the $i$-th iteration as: $\ell'_{i} = \psi_{i}(I_{raw}/\prod_{j = 0}^{i-1}\ell'_{j}; \omega_{i})$, where $\ell'_{i}$ is the output of the $i$-th stage $\psi_{i}$ and $\ell'_{0} = (1,1,1)$. The problem with this structure is that it is too heavy since it requires to optimize and store $i$ times more parameters than FC4, which makes it easy to overfit and far more redundant.


% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\columnwidth]{figures/compare}

%     \caption{Comparison with C4~\cite{yu2020c4}. The blocks in different colors mean their parameters are different.}

%     \label{fig:compare}
% \end{figure}


\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{IEEEtran/figures/isam.pdf}

    \caption{The detailed structure of the proposed Iteration-Specific Attention Module.}

    \label{fig:isam}
\end{figure}

Since all the stages in C4 always learn the same semantic features for the illuminant, and their only difference comes from the percentage among the color channels of the illuminant, we share the backbone in each stage of C4 and design an \textit{iteration-specific attention module} to re-calibrate the difference individually as shown in Figure~\ref{fig:nn}. The proposed framework has several advantages. 
First, sharing the backbone parameters helps us to build a compact model while obtaining better performance than C4. 
Second, since our network contains much fewer parameters, it is easier to be optimized than the original cascaded framework.
Finally, 
%based on our previous relighting analysis, 
the training combinations in different stages~(sub-networks) of C4 are different. For example, the $i$-th sub-network uses this combination $(I_{raw}/\prod_{j = 0}^{i-1}\ell'_{j}, \ell/\prod_{j = 0}^{ i-1}\ell'_{j})$ for training. However, in our shared sub-network, the shared backbone views more information than each of the sub-networks in C4 and its training combination is equivalent to the sum of the $M$-stages' combinations in C4:~$\sum_{i=1}^{M}(I_{raw}/\prod_{j = 0}^{i-1}\ell'_{j}, \ell/\prod_{j = 0}^{i-1}\ell'_{j})$. Obviously, this is a stronger data augmentation of relighting.

We also design a lightweight head for FC4 as our backbone~(L-FC4) which further reduces nearly 50\% of the parameters but gains better performance. Below, we give the details of the proposed \textit{iteration-specific attention module} and \textit{lightweight head}.

\textbf{Iteration-Specific Attention Module~(ISAM).}
 As discussed previously, ISAM aims to learn the color difference between stages using a lightweight structure. As shown in Figure~\ref{fig:isam}, the proposed attention block contains channel re-calibration and spatial re-calibration. In the channel re-calibration, inspired by the previous statistics-based gray-world~\cite{gray-world} and white-patch~\cite{white-patch}, we extract the global per-channel maximum and average values via global max pooling and global average pooling, respectively. Then, these features are learnt via two fully-connected layers. Finally, a sigmoid layer is used to re-calibrate the original features channel-wisely. The spatial re-calibration is similar to the channel re-calibration. Differently, we use channel-wise pooling for the features, and then a $7\times7$ convolutional layer and a sigmoid layer are used for the spatial feature learning and re-calibration. 
 As shown in Figure~\ref{fig:nn}, we insert multiple ISAMs with \textit{different} parameters before each max-pooling layer of the backbone except for the first one. 
The proposed ISAM is inspired by the widely-used attention modules~\cite{seblock,cbam} for image restoration~\cite{zamir2020cycleisp,liu2019dual} and high-level tasks~\cite{seblock,cbam}. However, to the best of our knowledge, for the first time, it is used as the \textit{iteration controller} in the cascaded framework.



\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{IEEEtran/figures/head.pdf}
    \caption{Comparison of parameters between the proposed lightweight head and the original head in FC4. Here, NL  represent Non-Local Block~\cite{non-local}.}
    \label{fig:head}
\end{figure}


\textbf{Lightweight Head.}
As shown in Figure~\ref{fig:head}, we also design a novel lightweight head to get a more compact backbone compared with the original FC4~\cite{hu2017fc4}. Specifically, besides the feature extraction from the first 12 layers of SqueezeNet, FC4 uses two convolutional layers, Conv6~(with $ 512\times64\times6\times6 $ parameters) and Conv7~(with $ 64\times3\times1\times1 $ parameters), to get the final global illumination. The Conv6 is designed to capture larger reception fields on high-level features, which is cumbersome and costs nearly 60\% of the parameters of the overall network. 
Thus, to reduce the parameters and also capture the long-range dependence, we design a lightweight head using a two-branch framework as shown in Figure~\ref{fig:nn}. In detail, in the local~(upper) branch, we reduce the original features spatially by $2\times2$ max pooling and then squeeze the original $512$ channels to $128$ by a $1\times1$ convolutional layer in order to work in a more compact space. Then, we estimate the long-range and global information via a non-local block~\cite{non-local}. After that, a 3-component prediction in the upper branch is generated by a $1\times1$ convolutional layer and global average pooling. We also design a global~(lower) branch by average pooling the original features globally. Then, two linear layers and a sigmoid layer are used to get another 3-component prediction in the lower branch. Finally, the predictions of these two branches are multiplied to generate the final illuminant with $L_2$ normalization for the current stage. The upper branch can be thought as white-patch localization, while the lower branch extracts the global information. This structure shows better performance and captures long-range dependencies as well, which has a negligible amount of parameters added to the backbone. 
%We compare the detailed structures between the proposed lightweight head FC4~(L-FC4) and the original FC4 in the supplementary materials.
%can also be considered as a global attention~\cite{seblock}.


% \begin{figure}[b]
%     \centering
%     \includegraphics[width=\columnwidth]{figures/MSHead}
%     \caption{The detailed structure of the proposed Multi-scale Head.}
%     \label{fig:mshead}
% \end{figure}


% We also notice a similar correct process has been used to create the multi-illumination benchmark~\cite{bianco2017single}, however, it has never been used and proved as data augmentation to stability the training in single illumination color constancy.
% \begin{table}[h]
%     \centering
%     \caption{Differences on training combinations.}
%     \begin{tabular}{l | l | c }
%     \toprule
%     Methods &  (input, label) & Sensor-aware? \\ \hline
%     Original  &  $ (I_{raw}, \ell) $ &  \\
%     FC4\cite{hu2017fc4}  &  $ (I_{raw}\times \xi, \ell \times \xi ) $ &  \\
%     % C4\cite{yu2020c4}  & FC4\cite{hu2017fc4} + $(I_{raw}/\prod_{j = 0, i-1}\ell'_{j}, \ell/\prod_{j = 0, i-1}\ell'_{j})$ \\
%     proposed & $( \frac{I_{raw}}{\ell} \times \ell', \ell')$ & \checkmark \\
%     \bottomrule
%     \end{tabular}
%     \label{tab:compare}
% \end{table}


\subsection{Loss Function}
\label{sec:loss}
Similar to C4~\cite{yu2020c4}, we use the multi-stage normalized angular loss as the objective. Specifically, for a network with $M$~($M=3$ in ~\cite{yu2020c4} and this paper) iterations~(stages), the  loss $\mathcal{L}$ is defined as:
\begin{equation}
    \mathcal{L} = \sum_{i=1}^{M} \frac{180}{\pi}\arccos({\frac{\ell \cdot \ell'_{i}}{\parallel \ell \parallel \parallel \ell'_{i} \parallel}}),
\end{equation}
where  $\ell'_{i} = \ell'_{i-1} \times \psi_{i}(I_{raw}/\ell'_{i-1})$ is the prediction of the $i$-th stage and $\ell'_{0} = (1,1,1)$ . 
%These losses guarantee the distribution of the predicted illumination in each stage, where the later stages use these illuminations for further relighting.
%In Gehler-Shi dataset, we also optimize the the hyper-parameters $\omega_{l}$ in each stages using~\cite{rloss}, which learn the hyper-parameters of each stage automatically for unbalanced dataset.



==> IEEEtran/subfiles/relatedwork.tex <==
\section{Related Work}
Existing methods on color constancy can be approximately categorized into two classes: traditional statistics-based and deep learning-based methods. Below, we give the detailed reviews of each part, while focusing on the discussions about recent works based on deep learning.

\subsection{Traditional Color Constancy}
%Color constancy has a long history in computer vision and color science.
Early methods estimate the scene illuminant using statistics features~\cite{bright-pixels,gray-index,gray-world, grey-pixel,white-patch,shades-of-gray} of the input image. Based on the assumption that the scene color is achromatic, the mean of each color channel~\cite{gray-world}, the gray edge~\cite{gray-edge} and the white patch~\cite{white-patch} are commonly used features for illumination estimation. Although these methods are simple and fast, the accuracy is unsatisfactory in real world prediction. To further boost the performance in real world scenes, machine learning-based methods show significantly better results than statistics-based methods. A branch of early works extract hand-crafted features~\cite{regression-tree,SVR} for learning, while the most recent works are all based on deep learning, which exhibits great potential in many computer vision tasks~\cite{alexnet,squeezenet,deng2009imagenet} including CC.

%, followed by a regressor, such as decision tree~\cite{regression-tree} or support vector regression~\cite{SVR}, which is used to regress the scene illumination. 
\subsection{Deep Color Constancy}

\textbf{Illumination Regression and Classification.} Since CC only needs to predict a global illumination, regression-based methods are easy to be applied. Bianco~\etal~\cite{bianco2015color} propose a patch-based network inspired by image classification~\cite{alexnet}. Then, Qiu~\etal~\cite{qiu2020color} design a feature re-weighted layer and use hierarchical features for regression. Besides a single patch, Xu~\etal~\cite{end2end} involve the triplet loss to constrain the differences among the patches from a single image. However, although illuminant can be simply regarded as a global feature, the low-level features, such as the white patch and gray edge, are also important. Besides regression, considering CC as a classification problem also draws attention from researchers~\cite{oh2017approaching,dsn,multi-hyp}. For example, \cite{multi-hyp} selects multiple candidates and weights them under a Bayesian framework. However, the selection of suitable candidates from the dataset hugely influences the performance and the accuracy is unsatisfactory.


\textbf{White Patch~(Point) Localization.} 
White patch has been shown to be highly connected to CC in statistics-based methods. Some works~\cite{ccc,ffcc,siie} extract a color $uv$-histogram in the log-chromatic space and then localize it following object detection. Differently, some recent fully convolutional neural network-based methods~\cite{hu2017fc4,yu2020c4} can also be considered as white-point localization ones. They extract features by neural networks directly using stronger backbones pre-trained on ImageNet~\cite{deng2009imagenet}. With the backbones, these methods have their novel structures, such as the confidence-weighted pooling layer~\cite{hu2017fc4}, to focus on the most related region automatically. Our proposed network also belongs to this category, but it obtains a more satisfactory accuracy with much fewer parameters.

%employ multiple illuminant hypotheses and then adaptively select or derive an estimate from the hypotheses.
% Learning-based methods estimate illuminant using a model learning from training data, which can be categorized into two classes by extracted feature: hand-crafted feature and learn-able feature. 

% Early work in this direction Learning-based works employ models trained on hand-crafted features extracted from the input image and utilize the extracted features by support vector regression~\cite{SVR}, regression tree~\cite{regression-tree}, \etc. 
%These methods based on hand-crafted features outperform those statistics-based a lot. 

%Later CNN-based methods are proved to be much more effect by make use of CNNs to learn better feature from inputs. CNN-based methods mainly contains two groups: gamut mapping learning \cite{siie} and directly regression learning~\cite{ccc,ffcc,hu2017fc4,dsn,cm,multi-hyp,mdlcc,yu2020c4,oh2017approaching,end2end}.  Afifi~\etal~\cite{siie} design a gamut mapping network to map the gamut of inputs into the canonical gamut, which contributes to sensor-independent, then estimate the illuminant from the latter gamut. The thought seems reasonable while its accuracy isn't  satisfactory. \cite{mdlcc} propose a camera-specific module to complete the goal of multi-domain learning and few-shot learning, but it has an disadvantage that needing lots of data from different devices when training. \cite{oh2017approaching,dsn,multi-hyp} employ multiple illuminant hypotheses and then adaptively select or derive an estimate from the hypotheses. \cite{ccc,ffcc} introduce 2-D uv-histograms in log-chromatic space to convert input images to histograms, then learn from the histograms to estimate illuminant. Compared to \cite{ccc,ffcc}, Convolutional Mean~\cite{cm} use only 3 conv-layers to estimate from input so that its model is very light and its performance is relatively fine. In \cite{hu2017fc4}, Hu \etal propose a Confidence-Weighted pooling method in the fully convolutional network named FC4 to cope with inputs with arbitrary size, which is actually an attention mechanism. Based on FC4~\cite{hu2017fc4}, Yu \etal \cite{yu2020c4} proposed a cascading color constancy structure named C4, which contributes to the state-of-the-art performance. Although C4~\cite{yu2020c4} make a surprising performance, the total amount of weights of C4 is three times larger than that that of FC4. Another state-of-the-art work~\cite{end2end} propose a deep illuminant network~(DIN) to extract semantic features and color features, and an illuminant-guided triplet network~(IGTN) as the regression network to estimate illuminant. 
%However with a backbone AlexNet~\cite{alexnet}, the model proposed by \cite{end2end} is too heavy to be applied on mobile devices.

\textbf{Pre-Training.} Unsupervised especially self-supervised learning draws extensive attention recently, which has been successfully utilized in image classification~\cite{moco,simclr} and natural languge processing~\cite{bert}. In CC, Lou~\etal~\cite{lou2015color} learn to minimize the loss between the network prediction and the labels obtained by a traditional statistic-based method on sRGB images. However, the results of the statistic-based method are inaccurate. Based on the fact that available sRGB images can be considered as white-balanced, Bianco and Cusano~\cite{bianco2019quasi} train their network to detect the achromatic patches by an achromatic loss. However, the heavy network and unsatisfactory performance restrict the usage of their method. Differently, our pre-training aims to regress the illuminant directly, which is simple and effective. Moreover, our pre-trained model can be also used for other state-of-the-art CC networks directly.

% \textbf{Data Augmentation}
% is a widely-used technique in deep learning to prevent overfitting and get better performance. Besides random cropping or resizing in image classification~\cite{alexnet}, many recent data augmentation methods are proposed to increase the diversity of training samples, such as synthesizing more realistic data by networks~\cite{wen2019single,cun2020towards,zamir2020cycleisp} and selecting augmentation policies by automatic machine learning~\cite{cubuk2019autoaugment,lim2019fast}. However, for color constancy, few methods are proposed to improve the training samples. In detail, Hu~\etal~\cite{hu2017fc4} relight the scene and illuminant by applying a random independent factor to each color channel for single-sensor color constancy. But this method breaks the color distribution of the particular sensor. Bani{\'c}~\etal~\cite{banic2019crop} photograph an all-color checker by a specific camera, and produce raw-space images by mapping normal sRGB images reversely. However, the reversed mapping ignores the complex camera pipeline and the authenticity of the produced images is also restricted by their lower~(five) bits approximation. Differently, 
% the proposed cross-sensor self-supervised per-taining aims to learn a cross-domain sensor-free model by illuminant simulation.

\textbf{Cross Sensor CC.}
The existence of CSS is the main reason why a model trained on one particular sensor is hard to be applied to another. Considering CSS, Gao~\etal~\cite{css} rectify the images from a source sensor and learn a model trained on a target sensor by mapped samples. Afifi~\etal~\cite{siie} design a gamut mapping network to map the gamut of inputs into the canonical gamut, which makes it sensor-independent, and estimate the illuminant from the latter gamut. The multi-hypothesis strategy~\cite{multi-hyp} aims at the cross-sensor evaluation by selecting the illuminant candidates on the target sensor data. Also, few-shot meta-learning~\cite{mcdonagh2018formulating} and multi-domain learning~\cite{mdlcc} are applied to CC to squeeze the gap among different domains. Differently, our method leverages the knowledge from larger-scale datasets by randomly sampling illuminants. 
%Different from previous works that discuss the effect of CSS on multiple domains, in this work, for the first time, we show how CSS can be used to improve the accuracy of illuminant estimation on a particular sensor.

\textbf{Compact Networks.}
Applying current deep learning models on resource-limited devices, such as mobile phones \cite{cheng2017survey,howard2017mobilenets,zhang2018shufflenet}, is a hot topic in the research community. In CC, although many previous networks~\cite{cm,ccc,ffcc,qiu2020color} are designed for lightweight structures and real-time prediction, the applicability of these methods is restricted by either a 
hand-crafted color $uv$-histogram~\cite{ccc,ffcc} or not-good-enough performance~\cite{cm,qiu2020color}. Differently, the proposed model is fully convolutional and obtains the state-of-the-art performance while using relatively fewer parameters.


==> subfiles/codeListingConfig.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%% CODE APPEARANCE CONFIG %%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%nicolas igor %%%%%%

%%%%%%%%%%%%%%%%% README %%%%%%%%%%%%%%%%%%%%
% This is a config file to set:
%   1. Style for listing package (could be use on any language)
%   2. Julia syntax highlighting definition
%   3. Command and environment to insert julia, python, and matlab code in your document easily.
%
%       a. new commands: \juliaFile, \pythonFile, and \matlabFile
%           All three are used like \juliaFile[folder_name]{file_name}
%           folder_name is optional, and do it with the slash, e.g. "myFolder/". When no folder is provided, it is assumed that the code is in the same directory as your document.
%           For file_name, do it without extension (it is assumed).
%       Example:
%           \juliaFile[codes/]{kMeans}
%           \juliaFile{randomForest}
%
%       b. new environments: if you want to write your code directly in your document. juliaText, pythonText, and matlabText are provided. Example:
%           \begin{juliaText}{Write your caption here.}
%           Write your code here
%           \end{juliaText}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



% Better font encoding, and customized fixed-width font
\usepackage[T1]{fontenc}
\usepackage{inconsolata}

% Colors Definition for Listing Highlighting 
\usepackage{color}
\definecolor{codeRed}{rgb}{0.5,0,0}
\definecolor{codeGreen}{rgb}{0,0.6,0}
\definecolor{codeBlue}{rgb}{0,0,0.5}
\definecolor{codeGray}{rgb}{0.5,0.5,0.5}
\definecolor{codeMauve}{rgb}{0.58,0,0.82}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%% LISTING FUN STARTS HERE!!! %%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{listings} % For displaying code

% General Appearance Settings in an Isolated Style
\lstdefinestyle{myStyle}{ %
  basicstyle=\small\ttfamily,      % the size of the fonts that are used for the code
  basewidth=0.5em,                 % sets size of reserved space on each column
  breakatwhitespace=true,          % sets if automatic breaks should only happen at whitespace
  breaklines=true,                 % sets automatic line breaking
  commentstyle=\color{codeGreen},  % comment style
  captionpos=b, 
  extendedchars=true,              % lets you use non-ASCII characters; for 8-bits encodings only, does not work with UTF-8
  frame=tb,	                       % adds a frame around the code
  keywordstyle=\color{codeBlue},       % keyword style
  numbers=left,                    % where to put the line-numbers; possible values are (none, left, right)
  numbersep=5pt,                   % how far the line-numbers are from the code
  numberstyle=\scriptsize\color{codeGray}, % the style that is used for the line-numbers
  rulecolor=\color{black},         % if not set, the frame-color may be changed on line-breaks within not-black text (e.g. comments (green here))
  showspaces=false,                % show spaces everywhere adding particular underscores; it overrides 'showstringspaces'
  showstringspaces=false,          % underline spaces within strings only
  showtabs=false,                  % show tabs within strings adding particular underscores
  stepnumber=1,                    % the step between two line-numbers. If it's 1, each line will be numbered
  numberfirstline=true, 
  numberblanklines=true,
  stringstyle=\color{codeMauve},     % string literal style
  tabsize=4,	                   % sets default tabsize to 4 spaces
}

% Definition of Julia Highlighting
\lstdefinelanguage{Julia}%
{ language = Matlab,% 
    keywordsprefix=\@,%
    morekeywords={
    exit,whos,edit,load,is,isa,isequal,typeof,tuple,ntuple,uid,hash,finalizer,convert,promote,
    subtype,typemin,typemax,realmin,realmax,sizeof,eps,promote_type,method_exists,applicable,
    invoke,dlopen,dlsym,system,error,throw,assert,new,Inf,Nan,pi,im,begin,while,for,in,return,
    break,continue,macro,quote,let,if,elseif,else,try,catch,end,bitstype,call,do,using,module,
    import,export,importall,baremodule,immutable,local,global,const,Bool,Int,Int8,Int16,Int32,
    Int64,Uint,Uint8,Uint16,Uint32,Uint64,Float32,Float64,Complex64,Complex128,Any,Nothing,nothing,
    function,type,typealias,abstract,case,false,otherwise,switch,true,include
  },%
  sensitive=true, %
  comment=[l]{\#}, % l is for line comment
  morecomment=[s]{\#=}{=\#}, % s is for start and end delimiter
  string=[b]" % defines that strings are enclosed in double quotes
}

% Command to include files of code easier, Julia
\newcommand{\juliaFile}[2][]{\lstinputlisting[caption=Script \emph{#2}., label=code:#2, style=myStyle, language=Julia]{#1#2.jl}}
% Command to include files of code easier, Python
\newcommand{\pythonFile}[2][]{\lstinputlisting[ label=code:#2, style=myStyle, language=Python]{#1#2.py}}
% Command to include files of code easier, Matlab
\newcommand{\matlabFile}[2][]{\lstinputlisting[caption=Script \emph{#2}., label=code:#2, style=myStyle, language=Matlab]{#1#2.m}}

% Environment to write by hand code easier, Julia
\lstnewenvironment{juliaText}[1]{\lstset{caption=#1, style=myStyle, language=Julia, firstnumber=1}}{}
% Environment to write by hand code easier, Python
\lstnewenvironment{pythonText}[1]{\lstset{caption=#1, style=myStyle, language=Python, firstnumber=1}}{}
% Environment to write by hand code easier, Matlab
\lstnewenvironment{matlabText}[1]{\lstset{caption=#1, style=myStyle, language=Matlab, firstnumber=1}}{}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%% LISTING FUN ENDED  %%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

